Combinations of Qualitative Winning for Stochastic Parity Games

We study Markov decision processes and turn-based stochastic games with parity conditions. There are three qualitative winning criteria, namely, sure winning, which requires all paths must satisfy the condition, almost-sure winning, which requires the condition is satisfied with probability~1, and limit-sure winning, which requires the condition is satisfied with probability arbitrarily close to~1. We study the combination of these criteria for parity conditions, e.g., there are two parity conditions one of which must be won surely, and the other almost-surely. The problem has been studied recently by Berthon et.~al for MDPs with combination of sure and almost-sure winning, under infinite-memory strategies, and the problem has been established to be in NP $\cap$ coNP. Even in MDPs there is a difference between finite-memory and infinite-memory strategies. Our main results for combination of sure and almost-sure winning are as follows: (a)~we show that for MDPs with finite-memory strategies the problem lie in NP $\cap$ coNP; (b)~we show that for turn-based stochastic games the problem is coNP-complete, both for finite-memory and infinite-memory strategies; and (c)~we present algorithmic results for the finite-memory case, both for MDPs and turn-based stochastic games, by reduction to non-stochastic parity games. In addition we show that all the above results also carry over to combination of sure and limit-sure winning, and results for all other combinations can be derived from existing results in the literature. Thus we present a complete picture for the study of combinations of qualitative winning criteria for parity conditions in MDPs and turn-based stochastic games.

==> background.tex <==
\section{Background}
\label{section:prelim}
\label{section:background}

For a countable set $S$ let $\dist{S}=\{d:S \rightarrow [0,1]~|~
\exists T\subseteq S \mbox{ such that } |T|\in \mathbb{N}, \forall
s \notin T ~.~ d(s)=0 \mbox{ and }\Sigma_{s\in T} d(s)=1\}$ be the set of
discrete probability distributions with finite support over $S$. 
A distribution $d$ is {\em pure} if there is some $s\in S$ such that
$d(s)=1$.

\paragraph{Stochastic Turn Based Games}
We give a short introduction to stochastic turn-based games.

A stochastic turn-based game is 
$G=(V,(V_0,V_1,V_p),E,\kappa)$, where $V$ is a finite set of
configurations, $V_0$, $V_1$, and $V_p$ form a partition 
of $V$ to \pzero, \pone, and stochastic configurations, respectively,
$E\subseteq V\times V$ is the set of 
edges, and $\kappa:V_p\rightarrow \dist{V}$ is 
a probabilistic transition for configurations in $V_p$ such that
$\kappa(v,v')>0$ implies $(v,v')\in E$.
If either $V_0=\emptyset$ or $V_1=\emptyset$ then $G$ is a Markov
Decision Process (MDP). If both $V_0=\emptyset$ and $V_1=\emptyset$
then $G$ is a Markov Chain (MC). If $V_p=\emptyset$ then $G$ is a
turn-based game (non-stochastic).
Given an MC $M$, an initial configuration $v$, and a measurable set
$W\subseteq V^\omega$, we denote by $\prob{M_v}{W}$ the measure of the
set of paths $W$.

A set of plays $W \subseteq V^\omega$ is a
\emph{parity} condition if there is a parity priority function
$\alpha:V\rightarrow \set{0,\ldots, d}$, with $d$ as its \emph{index},
such that a play $\pi=v_0,\ldots$ is in
$W$ iff $\min\{ c \in \set{0,\ldots, d} ~|~ \exists^\infty 
  i~.~\alpha(v_i)=c\}$ is even.
A parity condition $W$ where $d=1$ is a B\"uchi condition.
In such a case, we may identify the condition with the set
$B=\alpha^{-1}(0)$.
A parity condition $W$ where $d=2$ and $\alpha^{-1}(0)=\emptyset$ is a
co-B\"uchi condition.
In such a case, we may identify the condition with the set
$C=\alpha^{-1}(1)$. 

A \emph{strategy} $\sigma$ for \pzero is $\sigma:V^*\cdot V_0\rightarrow
\dist{V}$, such that $\sigma(w\cdot v)(v')>0$ implies $(v,v')\in E$.
A strategy $\pi$ for \pone is defined similarly.
A strategy is \emph{pure} if it uses only pure distributions.
A strategy uses memory $m$ if there is a domain $M$ of size $m$ and
two functions $\sigma_s:M\times V_0\rightarrow \dist{V}$ and
$\sigma_u:M\times V \rightarrow M$ such that for every $w\cdot v$ we have
$\sigma(w\cdot v)=\sigma_s(\sigma_u(w\cdot v),v)$, where
$\sigma_u(\epsilon)$ is some $m_0\in M$, and $\sigma_u(w\cdot
v)=\sigma_u(\sigma_u(w),v)$.
A strategy is memoryless if it uses memory of size $1$.
Two strategies $\sigma$ and $\pi$ for both players and an initial
configuration $v\in V$ induce a Markov chain
$v(\sigma,\pi)=(S(v),P,L,v)$, where $S(v)=\{v\}\cdot V^*$ and if $v\in
V_0$ we have $P(wv)=\sigma(wv)$, if $v\in V_1$ we have $P(wv)=\pi(wv)$
and if $v\in V_p$ then for every $w\in V^*$ and $v'\in V$ we have
$P(wv,wvv')=\kappa(v,v')$.

For a game $G$, an $\omega$-regular set of plays $W$, and a
configuration $v$,
the value $W$ from $v$ for \pzero, denoted $\val_0(W,v)$, and for
\pone, denoted $\val_1(W,v)$, 
are $$\val_0(W,v)=\ds\sup_{\sigma\in\Sigma}\ds\inf_{\pi\in\Pi}
\prob{v(\sigma,\pi)}{W}$$
and 
$$\val_1(W,v)=\ds\sup_{\pi\in\Pi}\ds\inf_{\sigma\in\Sigma}
\left (1-\prob{v(\sigma,\pi)}{W}\right ).$$
%We say that player $i$ wins $W$ \emph{almost surely} from $v$ if
%$\val_i(W,v)=1$. 
We say that \pzero wins $W$ \emph{surely} from $v$ if 
$\exists \sigma\in\Sigma~.~\forall \pi\in\Pi ~.~ v(\sigma,\pi)\subseteq
W$, where by $v(\sigma,\pi)\subseteq W$ we mean that \emph{all}
paths in $v(\sigma,\pi)$ are in $W$.
We say that \pzero wins $W$ \emph{almost surely} from $v$ if $\exists
\sigma\in\Sigma~.~\forall \pi\in\Pi ~.~ \prob{v(\sigma,\pi)}{W}=1$.
We say that \pzero wins $W$ \emph{limit surely} from $v$ if 
$\forall r<1~.~\exists\sigma\in\Sigma~.~\forall \pi\in\Pi ~.~ 
\prob{v(\sigma,\pi)}{W}\geq r$.
A strategy $\sigma$ for \pzero is optimal if
$\val_0(W,v)=\ds\inf_{\pi\in\Pi}\prob{v(\sigma,\pi)}{W}$. 

A game with condition $W$ is \emph{determined} if for every
configuration $v$ we have $\val_0(W,v)+\val_1(W,v)=1$.


\begin{theorem}
  Consider a stochastic two-player game $G$, an $\omega$-regular set
  of plays $W$, and a rational $r$.
  \begin{compactitem}
  \item
    For every configuration $v\in V$ we have
    $val_0(W,v)+val_1(W,v)=1$.
  \item
    If $G$ is finite and $W$ a parity condition, one can decide
    whether $val_i(W,v)\geq r$ in $\mbox{NP}\cap\mbox{co-NP}$ and
    $val_i(W,v)$ can be computed in exponential time
    {\rm \cite{CHJ04}}.
  \item
    If $W$ is a parity condition, 
    there is an optimal pure memoryless strategy $\sigma$ such that
    $\inf_{\pi\in\Pi}\prob{v(\sigma,\pi)}{W}=\val_0 (W,v)$
    {\rm \cite{CHJ04}}.
  \item
    If $G$ is a non-stochastic game then $\val_i(W,v)\in \{0,1\}$ for
    every $v \in V$ and there are optimal pure strategies for both
    players \cite{Tho90}.
  \item
    If $G$ is a non-stochastic game and $W$ is a parity condition,
    then whether $\val_i(W,v)=1$ can be decided in 
    UP$\cap$co-UP {\rm \cite{Jur98}}. Furthermore, the optimal
    strategies are memoryless {\rm \cite{Tho97}}.
  \item
    If $G$ is a non-stochastic game with $n$ configurations and $m$
    transitions and $W$ is a parity condition of index $d$ 
    then whether $\val_i(W,v)=1$ can be decided in
    time $O(n^{\log{d}+6})$ and if $d\leq \log{n}$ then in time
    $O(mn^{2.38})$ \cite{CJKLS17,JL17}.
  \item
    If $G$ is a non-stochastic game and $W$ is the intersection of two
    parity conditions, then whether $\val_i(W,v)=1$ can be
    decided in co-NP, whether $\val_i(W,v)=0$ can be decided in NP,
    and there is a finite-state optimal strategy for \pzero and a
    memoryless optimal strategy for \pone~{\rm \cite{CHP07}}.
  \end{compactitem}
  \label{theorem:pog determinacy}
  \label{theorem:pog complexity}
  \label{theorem:games complexity}
\end{theorem}


==> conc.tex <==
\section{Conclusions and Future Work}
\label{section:conclusions}
In this work we considered MDPs and turn-based stochastic games with 
two parity winning conditions, with combinations of qualitative 
winning criteria. 
In particular, we study the case where one winning condition must be 
satisfied surely, and the other almost-surely (or limit-surely).
We present results for MDPs with finite-memory strategies, and 
turn-based stochastic games with finite-memory and infinite-memory strategies.
Our results establish complexity results, as well as algorithmic results
for finite-memory strategies by reduction to non-stochastic games.
Some interesting directions of future work are as follows.
First, while our results establish algorithmic results for finite-memory 
strategies, whether similar results can be establishes for infinite-memory
strategies is an interesting open question.
Second, the study of beyond worst-case synthesis problem for turn-based 
stochastic games with quantitative objectives is another interesting 
direction of future work.



%%EARLIER QUESTIONS: 
%%1. Probabilistic vs deterministic. ANS: IN our case always deterministic is sufficient.
%%2. Bounded from 0 strategies. ANS: Not very interesting. Simple reach to SAS region. 





==> figures/gadget.tex <==
\game{
\po{1}{}{p_{as}(v)}
\labeln{1}{right=0.1mm of 1,xshift=-2mm,yshift=3mm}{$\overline{v}$}
\pz{2}{below of=1,xshift=-30mm}{p_{as}(v)}
\labeln{2}{left=0.1mm of 2}{$(\tilde{v} ,0)$}
\pz{3}{right of=2,xshift=7mm}{p_{as}(v)}
\labeln{3}{right=0.01mm of 3,xshift=-0.5mm,yshift=3mm}{$(\tilde{v} ,2)$}
\po{6}{below of=2}{0}
\labeln{6}{left=0.1mm of 6,xshift=0.5mm,yshift=2mm}{$(\hat{v} ,0)$}
\pz{7}{right of=6}{1}
\labeln{7}{right=0.1mm of 7,xshift=-0.5mm,yshift=2mm}{$(\hat{v} ,1)$}
\po{8}{right of=7}{2}
\labeln{8}{right=0.1mm of 8,xshift=-0.5mm,yshift=2mm}{$(\hat{v} ,2)$}
\pz{9}{right of=8}{3}
\labeln{9}{right=0.1mm of 9,xshift=-0.7mm,yshift=2mm}{$(\hat{v} ,3)$}
\po{10}{right of=9}{4}
\labeln{10}{right=0.1mm of 10,xshift=-0.5mm,yshift=4mm}{$(\hat{v} ,4)$}
\pz{4}{above of=9,xshift=7mm}{p_{as}(v)}
\labeln{4}{left=0.1mm of 4,xshift=0.5mm,yshift=-2mm}{$(\tilde{v},4)$}
\node (s1) [right=2mm of 4] {$\cdot$};
\node (s2) [right=2mm of s1] {$\cdot$};
\node (s3) [right=2mm of s2] {$\cdot$};
\node (s6) [right=3mm of 10] {$\cdot$};
\node (s7) [right=2mm of s6] {$\cdot$};
\node (s8) [right=2mm of s7] {$\cdot$};
\pz{5}{right of=s3}{p_{as}(v)}
\labeln{5}{right=0.1mm of 5,xshift=-7mm,yshift=6mm}{$(\tilde{v},p_{as}(v){+}1)$}
% Remove the p_{as}(v)+1 node
\pz{11}{below of=5}{p_{as}(v)}
%\pz{11}{below of=5,xshift=-7mm}{p_{as}(v)}
\labeln{11}{left=0.1mm of 11,xshift=1mm,yshift=-3mm}{$(\hat{v},p_{as}(v))$}
%\po{12}{right of=11}{\tiny p_{as}(v){+}1}
%\labeln{12}{right=0.1mm of 12,xshift=-8mm,yshift=5mm}{$(\hat{v},p_{as}(v){+}1)$}

\edgestosucc{6}
\edgestosucc{7}
\edgestosucc{8}
\edgestosucc{9}
\edgestosucc{10}
\edgestosucc{11}
% Remove the p_{as}(v)+1 node
%\edgestosucc{12}

% This is the draft for edges to succ macro:
%\node (ls1) [below of=6,yshift=2mm] {$succ(v)$};
%\node (ls1r) [right=0.1mm of ls1,yshift=-2mm] {};
%\node (ls1l) [left=0.1mm of ls1,yshift=-2mm] {};
%\edge{6}{ls1r}
%\edge{6}{ls1l}

\edge{1}{2}
\edge{1}{2}
\edge{1}{3}
\edge{1}{4}
\edge{1}{5}
\edge{2}{6}
\edge{3}{7}
\edge{3}{8}
\edge{4}{9}
\edge{4}{10}
\edge{5}{11}
% Remove the p_{as}(v)+1 node
%\edge{5}{12}
}


==> figures/mdp.tex <==
  \game{
    \pz{1}{}{l}
    \labeln{1}{left=0.1mm of 1,xshift=1mm,yshift=3mm}{$(0,2)$}
    \pp{2}{right of=1}{p}
    \labeln{2}{left=0.1mm of 2,xshift=7mm,yshift=10mm}{$(1,2)$}
    \pz{3}{right of=2}{c}
    \labeln{3}{left=0.1mm of 3,xshift=7mm,yshift=-5mm}{$(1,2)$}
    \pz{4}{right of=3}{r}
    \labeln{4}{right=0.1mm of 4,xshift=1mm,yshift=3mm}{$(0,1)$}
    \fulledge{1}{3}{}{bend right}{}
    \fulledge{2}{1}{$\frac{1}{2}$}{}{xshift=2mm,yshift=6mm}
    \fulledge{2}{3}{$\frac{1}{2}$}{bend left}{xshift=-3mm,yshift=-1mm}
    \fulledge{3}{2}{}{}{}
    \fulledge{3}{4}{}{}{}
    \fulledge{4}{3}{}{bend left}{}
  }


==> figures/sls.tex <==
\game{
\pz{1}{}{l}
\labeln{1}{left=0.1mm of 1,xshift=1mm,yshift=3mm}{$(0,1)$}
\pz{2}{right of=1}{c}
\labeln{2}{left=0.1mm of 2,xshift=7mm,yshift=-5mm}{$(1,1)$}
\pp{3}{right of=2}{p}
\labeln{3}{left=0.1mm of 3,xshift=7mm,yshift=-5mm}{$(1,1)$}
\pz{4}{right of=3}{r}
\labeln{4}{right=0.1mm of 4,xshift=0mm,yshift=3mm}{$(0,0)$}
\fulledge{1}{1}{}{loop above}{}
\fulledge{2}{1}{}{}{}
\fulledge{2}{3}{}{}{}
\fulledge{3}{2}{$\frac{1}{2}$}{bend right}{yshift=6mm}
\fulledge{3}{4}{$\frac{1}{2}$}{}{}
\fulledge{4}{4}{}{loop above}{}
}


==> intro.tex <==
\section{Introduction}
\label{section:intro}


\noindent{\em Stochastic games and parity conditions.}
Two-player games on graphs are an important model to reason about 
reactive systems, such as, reactive synthesis~\cite{Chu63,PR89a},
open reactive systems~\cite{AHK02}.
To reason about probabilistic behaviors of reactive systems, such games
are enriched with stochastic transitions, and this gives rise to models
such as Markov decision processes (MDPs)~\cite{FV97,Puterman} and turn-based 
stochastic games~\cite{Con92}. 
While these games provide the model for stochastic reactive systems, 
the specifications for such systems that describe the desired non-terminating 
behaviors are typically $\omega$-regular conditions~\cite{Tho90}.
The class of parity winning conditions can express all $\omega$-regular 
conditions, and has emerged as a convenient and canonical form of 
specification for algorithmic studies in the analysis of stochastic reactive 
systems.





\smallskip\noindent{\em Qualitative winning criteria.} 
In the study of stochastic games with parity conditions, 
there are three basic qualitative winning criteria, namely,
(a)~{\em sure winning}, which requires all possible paths to satisfy
the parity condition; 
(b)~{\em almost-sure winning}, which requires the parity condition to
be satisfied with probability~1; and  
(c)~{\em limit-sure winning}, which requires the parity condition to
be satisfied with probability arbitrarily close to~1. 
For MDPs and turn-based stochastic games with parity conditions, almost-sure winning coincide with limit-sure 
winning, however, almost-sure winning is different from sure winning~\cite{Cha07}.
Moreover, for all the winning criteria above, if a player can ensure winning, she can do so 
with memoryless strategies, that do not require to remember the past history of the game.
All the above decision problems belong to NP $\cap$ coNP, and the 
existence of polynomial-time algorithm is a major open problem.


\smallskip\noindent{\em Combination of multiple conditions.} 
While traditionally MDPs and stochastic games have been studied with a
single condition with respect to  
different winning criteria, in recent studies combinations of winning criteria has emerged
as an interesting problem. 
An example is the {\em beyond worst-case synthesis} problem that combines 
the worst-case adversarial requirement with probabilistic guarantee~\cite{BFRR17}. 
Consider the scenario that there are two desired conditions, one of which is 
critical and cannot be compromised at any cost, and hence sure winning must 
be ensured, whereas for the other condition the probabilistic behavior can 
be considered. 
Since almost-sure and limit-sure provide the strongest probabilistic guarantee, 
this gives rise to stochastic games where one condition must be satisfied 
surely, and the other almost-surely (or limit-surely). 
This motivates the study of different conditions with different qualitative 
winning criteria, which has been already studied for MDPs with parity conditions in~\cite{BRR17}.


\begin{table*}[tb]
% \vspace{-4mm}
\renewcommand{\arraystretch}{1.1}
\caption{Summary of Results for Sure-Almost-sure as well as Sure-Limit-sure Winning for Parity Conditions. New results are boldfaced. The reductions give algorithmic 
results from algorithms for non-stochastic games.}\label{tab1}
\vspace{-4mm}
\centering
\begin{tabular}{@{}|l|c|c|@{}}
\hline 
Model & Finite-memory  & Infinite-memory\\
\hline
MDPs  & {\bf NP $\cap$ coNP} & NP $\cap$ coNP~\cite{BRR17} \\
      & {\bf Reduction to non-stochastic parity games} & \\
 \hline 
Turn-based   & {\bf coNP-complete} & {\bf coNP-complete} \\
stochastic game      & {\bf Reduction to non-stochastic games} & \\
                     & {\bf with conjunction of parity conditions} & \\
 \hline
\end{tabular}
\vspace{-4mm}
\end{table*}



\begin{table}[tb]
\renewcommand{\arraystretch}{1.1}
\caption{Conjunctions of various qualitative winning criteria.}\label{tab2}
\vspace{-4mm}
\centering
\begin{tabular}{@{}|c|c|c|@{}}
\hline 
Criteria 1 & Criteria 2  & Solution Method\\
\hline
Sure $\psi_1$ & Sure $\psi_2$ & Sure $(\psi_1 \land \psi_2)$ \\
Sure $\psi_1$ & Almost-sure $\psi_2$ & This work \\
Sure $\psi_1$ & Limit-sure $\psi_2$ & This work \\
Almost-sure $\psi_1$ & Almost-sure $\psi_2$ & Almost-sure $(\psi_1 \land \psi_2)$ \\
Almost-sure $\psi_1$ & Limit-sure $\psi_2$ & Almost-sure $(\psi_1 \land \psi_2)$ \\
Limit-sure $\psi_1$ & Limit-sure $\psi_2$ & Almost-sure $(\psi_1 \land \psi_2)$ \\
\hline 
\end{tabular}
\vspace{-8mm}
\end{table}

\smallskip\noindent{\em Previous results and open questions.}
While MDPs and turn-based stochastic games with parity conditions have been widely 
studied in the literature (e.g.,~\cite{CY95,EKVY08,BK08b,CJH03,CJH04,Cha07}), 
the study of combination of different qualitative winning criteria is recent. 
The problem has been studied only for MDPs with sure winning criteria for one parity condition, 
and almost-sure winning criteria (also probabilistic threshold guarantee) for another parity condition,
and it has been established that even in MDPs infinite-memory strategies are required, and 
the decision problem lies in NP $\cap$ coNP~\cite{BRR17}. 
While the existence of infinite-memory strategies represent the general theoretical problem, 
an equally important problem is the existence of finite-memory strategies, as the class of 
finite-memory strategies correspond to realizable finite-state transducers 
(such as Mealy or Moore machines). 
The study of combination of qualitative winning criteria for parity conditions is open 
for MDPs with finite-memory strategies, and turn-based stochastic games with both infinite-memory
and finite-memory strategies. 
In this work we present answers to these open questions.


\smallskip\noindent{\em Our results.} In this work our main results are as follows:
\begin{compactenum}
\item For MDPs with finite-memory strategies, we show that the combination of sure winning and 
almost-sure winning for parity conditions also belong to NP $\cap$ coNP, and we present 
a linear reduction to parity games.
Our reduction implies a quasi-polynomial time algorithm, and also polynomial time algorithm 
as long as the number of indices for the sure winning parity condition is logarithmic. 
Note that no such algorithmic result is known for the infinite-memory case for MDPs.

\item For turn-based stochastic games, we show that the combination of sure and almost-sure winning 
for parity conditions is a coNP-complete problem, both for
finite-memory as well as infinite-memory strategies. 
For the finite-memory strategy case we present a reduction to
non-stochastic games with conjunction of parity conditions, which
implies a fixed-parameter tractable algorithm, as well as a
polynomial-time algorithm as long as the number of indices of the
parity conditions are logarithmic.

\item Finally, while for turn-based stochastic parity games
  almost-sure and limit-sure winning coincide, 
we show that in contrast, while ensuring one parity condition surely,
limit-sure winning does not  
coincide with almost-sure winning even for MDPs.
However, we show that all the above results established for
combination of sure and almost-sure winning  
also carries over to sure and limit-sure winning.

\end{compactenum}
Our main results are summarized in Table~\ref{tab1}. 
In addition to our main results, we also argue that our results complete the picture of all 
possible conjunctions of qualitative winning criteria as follows:
(a)~conjunctions of sure (or almost-sure) winning with conditions $\psi_1$ and $\psi_2$ is equivalent 
to sure (resp., almost-sure) winning with the condition $\psi_1 \land \psi_2$ (the conjunction of the conditions);
(b)~by determinacy and since almost-sure and limit-sure winning coincide for $\omega$-regular conditions,
if the conjunction of $\psi_1 \land \psi_2$ cannot be ensured almost-surely, then the opponent can ensure
that at least one of them is falsified with probability bounded away from zero; and thus conjunction of 
almost-sure winning with limit-sure winning, or conjunctions of limit-sure winning coincide with 
conjunction of almost-sure winning.
This is illustrated in Table~\ref{tab2} and shows that we present a complete picture of 
conjunctions of qualitative winning criteria in MDPs and turn-based stochastic games.
 






\smallskip\noindent{\bf Related works.}
We have already mentioned the most important related works above.
We discuss other related works here.
MDPs with multiple Boolean as well as quantitative objectives have been widely studied 
in the literature~\cite{CMH06,EKVY08,FKN11,BBCFK11,CKK15}.
For non-stochastic games combination of various Boolean objectives is conjunction of the objectives,
and such games with multiple quantitative objectives have been studied in the literature~\cite{VCDHRR15,CDRR15}.
For turn-based stochastic games, the general analysis of multiple quantitative objectives is 
intricate, and they have been only studied for special cases, such as, reachability objectives~\cite{CFKSW13}
and almost-sure winning~\cite{BKTW15,CD16}.
However none of these above works consider combinations of qualitative winning criteria.
The problem of beyond worst-case synthesis has been studied for MDPs 
with various quantitative objectives~\cite{BFRR17,RRS15}, such as long-run average, shortest path,
and for parity objectives~\cite{BRR17}.
We extend the literature of the study of beyond worst-case synthesis problem 
for parity objectives by considering turn-based stochastic games and the distinction
between finite-memory and infinite-memory strategies.




%{\bf OLD THOUGHTS:}
%Two-player games are an important model to reason about strategies and 
%The analysis of two-player games and MDPs are used in many
%verification, and synthesis cases in order to reason
%about the options and strategies avaialble.
%Traditionally, these constructs have been considered with quailtative
%(i.e., Boolean) winning conditions corresponding to correctness or
%fulfillment of specifications.
%The parity winning condition has arisen as an expressive and
%convenient tool for algorithmic analysis of omega-regular conditions.
%In recent years, the limitations of this approach have started to
%emerge and it has become clear that in some cases a quantitative
%approach is required.

%mean-payoff
%discounted-sum
%more general games with probabilities

%But in many cases, the combination of multiple conditions are
%required.
%For example, how 


==> sas.tex <==
\section{Sure-Almost-Sure Parity Games}
\label{section:sas games}

We now turn our attention to sure-almost-sure parity games, which have 
not been considered in \cite{BRR17}.
We have already established the difference between finite and infinite
memory for \pzero even for MDPs.
We first show that sure-almost-sure games are determined.
Then, considering the decision of winning, we show for \pone
memoryless strategies are sufficient.
It follows that her winning is NP-complete.
We show that deciding whether \pzero has a (general) winning strategy 
is co-NP-complete.
Finally, we show that the case of finite memory (for \pzero) can be 
solved by a reduction to (non-stochastic) two-player games.

A sure-almost-sure (SAS) parity game is
$G=(V,(V_0,V_1,V_p)$, $E,\kappa,\mathcal{W})$, 
where all components are as before and $\mathcal{W}$ consists of
\emph{two} parity conditions $W_s\subseteq V^\omega$ and
$W_{as}\subseteq V^\omega$.
Strategies and the resulting Markov chains are as before.
We say that \pzero wins $G$ from configuration $v$ if she has a
strategy $\sigma$ such that for every strategy $\pi$ of \pone we have
$v(\sigma)\subseteq W_s$ and 
$\prob{v(\sigma,\pi)}{W_{as}}=1$.
That is, \pzero has to win for sure (on all paths) with respect to
$W_s$ and with probability $1$ with respect to $W_{as}$.


\subsection{Determinacy}
We start by showing that SAS parity games are determined.

\begin{theorem}
  SAS parity games are determined.
  \label{theorem:sas games determinacy}
\end{theorem}

\newcommand{\proofoftheoremsasgamesdeterminacy}{
\begin{proof}
  We define a Martin-like reduction that annotates configurations with
  the values that \pzero can get from them according to $W_{as}$
  \cite{Mar98}.
  Formally, we have the following.
  Let $G=(V,(V_0,V_1,V_p), E,\kappa,\mathcal{W})$.
  We define the following two-player game:
  Let $G'=(V',(V'_0, V'_1), E', \mathcal{W}')$, where $G'$ has the
  following components:
  \begin{itemize}
  \item
    The set of configurations $V' = V'_0 \cup V'_1$, where
    $V'_0 = \{ (v,r) ~|~ v\in V \mbox{ and } r\in [0,1)\}$ and 
    $V'_1 = \{ (v,f) ~|~ v\in V \mbox { and } f:succ(v) \rightarrow
      ([0,1)\cup \{\bot\})\}$
  \item
    The transitions of $G'$ are as follows.
    $$
    \begin{array}{l l r}
    E = &
    \left \{ ((v,r),(v,f)) ~\left |
    \begin{array}{l}
      v\in V_0,~ \exists w\in succ(v)~.~
      f(w)\neq \bot\\
      \mbox{and } f(w)\geq r 
    \end{array}
    \right. \right \}& \cup \\
    &
    \left \{ ((v,r),(v,f)) ~\left |
    \begin{array}{l}
      v\in V_1,~ \forall w\in succ(v)~.~
      f(w) \neq \bot \\
      \mbox{and } f(w) \geq r
    \end{array} \right . \right \} &
    \cup \\
    &
    \left \{ ((v,r),(v,f)) \left |
    \begin{array}{c}
      v\in V_p, \forall w \in succ(v) ~.~f(w)\neq \bot \\
      \mbox{and }
      \sum_{w\in succ(v)} \kappa(v,w)\cdot f(w) \geq r
      \end{array} \right. \right \}
      & \cup \\
     & \{ ((v,f),(w,f(w))) ~|~ w\in succ(v) \mbox{ and } f(w) \neq
    \bot \}
    \end{array}
    $$
  \item
    The winning condition is:
    $$
    \begin{array}{l c l c}
      W' & = &
      \{ w ~|~ w \in (V\times (0,1))^* \cdot (V\times \{0\})^\omega
      \mbox{ and } w\Downarrow_V \in W_{s}\} & \cup\\
      & &
      \{ w ~|~ w\in (V\times (0,1))^\omega \mbox{ and }
      w\Downarrow_V\in W_s \cap W_{as}\}
      \end{array}
      $$
  \end{itemize}
  That is, every configuration is annotated by the value that \pzero
  can win from it according to $W_{as}$. Then, \pzero chooses a
  function that shows what the value is for the successors of $v$
  followed by a choice of \pone of which successor to follow.
  In configurations in $V_0$, \pzero is allowed to use $\bot$ to some
  successors to signify that she has to win from at least one
  successor.
  In configurations in $V_1$, \pzero must choose numerical values for
  all successors. She must choose a value larger than current value
  for all of them. Indeed, if the value is lower than current value
  for one of them \pone would choose that successor and win.
  In configurations in $V_p$, \pzero must choose numerical values for
  all successors. The weighted average of the values of successors
  must be at least the current value. This means that some successors
  can have the value $0$.
  If the value is $0$, \pzero still needs to win according to
  $W_s$. That is, the game proceeds with the value $0$ forever.
  If the value is non-zero, she needs to show that she can win
  according to $W_s$ and obtain that value for the measure of winning
  paths according to $W_{as}$.

  This is a turn-based two-player game (albeit somewhat large) and as
  such is determined \cite{Mar75}.
  Let $W'_0$ be the set of configurations winning for \pzero in $G'$.
  We show that $v$ is winning for \pzero in $G$ iff
  $\{v\}\times [0,1) \subseteq W'_1$.
  That is, \pzero wins from $(v,r)$ for every possible value of $r$
  (note that $1$ is not a possible value of $r$).

  Suppose that \pzero wins from $(v,r)$ for every $r\in [0,1)$.
  It follows that for every $\epsilon >0$ there is a strategy of
  \pzero winning from $(v,1-\epsilon)$.
  All the plays consistent with this strategy are winning according to
  $W_s$.
  According to Martin's proof \cite{Mar98} the measure of plays
  winning for \pzero for $W_{as}$ is at least $1-\epsilon$.
  The two together show that \pzero wins from $v$.

  Suppose otherwise, then there is some value $r$ such that \pone wins
  from $(v,r)$ in $G'$.
  If $r=0$, then the strategy of \pone in $G'$ can be used to show
  that \pone wins according to the winning condition $W_s$.
  If $r\neq 0$ then Martin's proof can be used to show
  that \pone has a strategy that forces the measure of plays not in
  $W_{as}$ to be at least $1-r>0$.
\end{proof}
}

\shorten{
  \proofoftheoremsasgamesdeterminacy
}{
  In Appendix we prove that a reduction similar to Martin's proof that
  Blackwell games are determined by reducing them to turn-based
  two-player \cite{Mar98} games shows determinacy also for SAS games.
}

\subsection{General Winning}

We show that determining whether \pzero has a (general) winning
strategy in an SAS parity game is co-NP-complete and that for \pone
finite-memory strategies are sufficient and that deciding her winning
is NP-complete.


\begin{theorem}
  In an SAS parity game memoryless strategies are sufficient for
  \pone.
  \label{theorem:sas games memoryless player one}
\end{theorem}

\newcommand{\proofoftheoremsasgamesmemorylessplayerone}{
\begin{proof}
  WLOG we consider that every \pone-configuration $v$ has two successors
  $v_a$ and $v_b$: if $v$ has one successor it can be considered as \pzero-configuration;
  and the case where there are more than two successors can be reduced to
  the case of two successors by adding more configurations for \pone.
  We prove the result by induction on the number of configurations
  controlled by \pone.
  This technique has used in the context of non-stochastic games~\cite{GZ05}, as well
  as stochastic games~\cite{GK14,CD16}, but only for single objectives, whereas 
  we use it for combination of qualitative criteria. 


  If there are no configurations controlled by \pone then clearly a
  memoryless strategy suffices for her.
  Assume by induction that in a game with less than $k$ configurations
  controlled by \pone she can win with memoryless strategies.
  Consider a game with $k$ configurations in $V_1$.
  Let $v$ be such a configuration that has two successors $v_a$ and $v_b$.
  Let $G_a$ be the game $G$ where the edge from $v$ to $v_b$ is
  removed and let $G_b$ be the game $G$ where the edge from $v$ to
  $v_a$ is removed.
  Assume that \pone wins in $G$ but requires memory to do so.
  It follows that \pone cannot win both $G_a$ and $G_b$, otherwise,
  by induction, she would have a memoryless winning strategy and the
  same strategy would be extended to a memoryless winning strategy in
  $G$.
  It follows that \pzero has winning strategies $\sigma_a$ and
  $\sigma_b$ in $G_a$ and $G_b$, respectively.
  We compose $\sigma_a$ and $\sigma_b$ to a winning strategy in $G$.
  \pzero starts playing according to $\sigma_a$.
  Considering a history $h=v_0\cdots v_n$, $h$ can be partitioned to
  $h_0,h_1,\ldots,h_k$, where for every $i$ the last configuration of
  $h_i$ is $v$ and $v$ does not appear elsewhere in $h_i$.
  Let $h_a$ be the restriction of $h$ to those $h_i$ such that $v_b$
  is not the first configuration in $h_i$ (including $h_0$).
  Let $h_b$ be the restriction of $h$ to those $h_i$ such that $v_b$
  is the first configuration in $h_i$ (excluding $h_0$).
  Then, the strategy $\sigma$ in $G$ plays according to $\sigma_a$ if
  the last move from $v$ was to $v_a$ (or $v$ has not been visited)
  and according to $\sigma_b$ if the last move from $v$ was to $v_b$.
  When playing according to $\sigma_a$ the strategy $\sigma$ considers
  the history $h_a$ and whenever playing according to $\sigma_b$ the
  strategy $\sigma$ considers the history $h_b$.
  It follows that $\sigma$ is well defined.

  Consider a play $r$ consistent with $\sigma$. Clearly, $r$ can be
  partitioned to $r_0,\ldots$ according to the visits to $v$ similar
  to the way a history is partitioned and to the projections $r_a$ and
  $r_b$.
  Then, $r_a$ and $r_b$ are plays in $G_a$ and $G_b$ consistent with
  $\sigma_a$ and $\sigma_b$.
  It follows that $r_a$ and $r_b$ are winning for \pzero according to
  $W_s$.
  As $W_s$ is a parity condition the minimum parity occurring
  infinitely often in $r_a$ is even and the minimum parity occurring
  in $r_b$ is even.
  It follows that the minimal parity occurring infinitely often in $r$
  is even and it is winning according to $W_s$.

  Given a strategy for \pone and the resulting Markov chain
  $w(\sigma,\pi)$ we can consider the same partition to
  $w_a(\sigma,\pi)$ and $w_b(\sigma,\pi)$ of the Markov chains.
  The Markov chain $w_a(\sigma,\pi)$ is consistent with $\sigma_a$ and
  $w_b(\sigma,\pi)$ is consistent with $\sigma_b$.
  It follows that the probability of winning according to $W_{as}$ is
  1 in both $w_a(\sigma,\pi)$ and $w_b(\sigma,\pi)$.

  The shuffle of two plays $r_1$ and $r_2$ is a play
  $r=u_0,u_1,\ldots$, where $u_i\in V^*$ and $r_1=u_0\cdot u_2\cdots$
  and $r_2=u_1\cdot u_3\cdots$.
  A winning condition is shuffle closed if for every two plays
  $r_1,r_2\in W$ we have that every shuffle $r$ is in $W$ as well.
  Clearly, parity condition is shuffle closed.
  For shuffle-closed winning conditions we know that
  $$\prob{w(\sigma,\pi)}{W_{as})} \geq \min
  (\prob{w_a(\sigma,\pi)}{W_{as}},\prob{w_b(\sigma,\pi)}{W_{as}}).$$
  As $\sigma_a$ and $\sigma_b$ are winning it follows that
  $\prob{w_a(\sigma,\pi)}{W_{as}}=1$,
  $\prob{w_b(\sigma,\pi)}{W_{as}}=1$ and
  $\prob{w(\sigma,\pi)}{W_{as})}\geq 1$.
\end{proof}
}

\shorten{
  \proofoftheoremsasgamesmemorylessplayerone
}{
  In Appendix we show by an inductive argument over the number of
  configurations of \pone (similar to that done in
  \cite{GZ05,GK14,CD16}) that \pone has a memoryless optimal strategy.
}

\begin{corollary}
    Consider an SAS parity game.
    Deciding whether \pone wins is NP-complete and whether \pzero wins
    is co-NP-complete.
  \label{corollary:complexity of sas games}
\end{corollary}

\begin{proof}
  Consider the case of \pone.
  Membership in NP follows from guessing the (memoryless) winning
  strategy of \pone in $G$.
  The result is an MDP whose winning can be reduced to a parity game
  of polynomial size as we have shown in Section~\ref{section:sas
    MDPs}.
  It follows that winning for \pone in such an MDP can be determined
  in NP.
  An algorithm would guess the two strategies simultaneously and
  check both in polynomial time over the resulting Markov chain.

  Hardness follows from considering SAS games with no stochastic
  configurations \cite{CHP07}.

  Consider the case of \pzero.
  Membership in co-NP follows from dualizing the previous argument
  about membership in NP and determinacy.

  Hardness follows from considering SAS games with no stochastic
  configurations \cite{CHP07}.
\end{proof}

\subsection{Winning with Finite Memory}

We show that in order to check whether \pzero can win with finite
memory it is enough to use the standard reduction from almost-sure
winning in two-player stochastic parity games to sure winning in
two-player parity games \cite{CJH04}.

\begin{theorem}
  In a finite SAS parity game with $n$ locations and $d_{as}$
  almost-sure index deciding whether a node $v$ is winning for \pzero
  with finite memory can be decided by a reduction to a two-player
  game with $O(n\cdot d_{as})$ locations, where the winning condition
  is an intersection of two parity conditions of the same indices.
%  and whether a configuration $v$ is winning for
%    \pone is NP-complete.
  \label{theorem:sas games finite memory}
\end{theorem}

% Proof of lemma good ranking induces
% the proof is here as newcommand inside a proof environment
% does not work
\newcommand{\proofoflemmagoodrankinginduces}{
  \begin{proof}
    Let $\epsilon$ be the minimal probability of a transition in
    $G$.
    As $G$ is finite $\epsilon$ exists. 
    For configurations in $V_0\cup V_1$ the definitions of good parity
    ranking and almost-sure ranking coincide.
    
    Consider a configuration $v\in V_p$ and the matching
    configuration $\overline{v}$. 
    Let $p=p_{as}(v)$. Consider the appearance of $(v,m)$ in
    $G\times M$ and $(\overline{v},m)$ in $G'\times M$ for some
    memory value $m$.
    We consider the cases where $p$ is even and when $p$ is odd.
    \begin{itemize}
    \item
      Suppose that $p$ is even.
      If there is some minimal $i$ such that the choice of
      $\sigma'_0$ from $((\tilde{v},2i),m')$ in $G'\times M$ is
      $((\hat{v},2i-1),m'')$.
      Then, there is some $w\in succ(v)$ and some $m'''$ such that
      $$\vec{r}(w,m''')<_{2i-1}\vec{r}((\hat{v},2i-1),m'') \leq_{p}
      \vec{r}((\tilde{v},2i),m')\leq_p \vec{r}(\overline{v},m).$$
      It follows that $\prob{v}{\vec{r}_{<_{2i-1}}}\geq \epsilon$.
      Furthermore, as $i$ is minimal it follows that $i\neq 0$ and
      that the choice of $\sigma'_0$ from $((\tilde{v},2i-2),n)$ is
      $((\hat{v},2i-2),n')$, which belongs to \pone in $G'\times M$.
      Then, for every successor $(w,n''')$ of $((\hat{v},2i-2),n')$ we
      have
      $$\vec{r}(w,n''') \leq_{2i-2} \vec{r}((\hat{v},2i-2),n'') \leq_p
      ((\tilde{v},2i-2),n') \leq_p (\overline{v},m).$$
      It follows that $\prob{v}{\vec{r}_{\leq_{2i-2}}}\geq 1$.
      
      If there is no such $i$, then the choice of $\sigma'_0$ from
      $((\tilde{v},p),m')$ in $G'\times M$ is $((\hat{v},p),m'')$
      and for every $w\in\succ(v)$ there is some $m'''$ such that
      $$\vec{r}(w,m''') \leq_p \vec{r}((\hat{v},p),m'') \leq_p
      \vec{r}((\tilde{v},p),m') \leq_p \vec{r}(\overline{v},m).$$
      If follows that $\prob{v}{\vec{r}_{\leq_p}}\geq 1$. 
    \item
      Suppose that $p$ is odd.
      In this case there must be some minimal $i$ such that the
      choice of $\sigma'_0$ from $((\tilde{v},2i),m')$ is
      $((\hat{v},2i-1),m'')$.
      We can proceed as above.
    \end{itemize}
  \end{proof}
}

% Proof of lemme good as ranking induces
% The proof is here as newcommand inside a proof environment
% does not work
\newcommand{\proofoflemmagoodasrankinginduces}{
  \begin{proof}
    The conditions for parity ranking and almost-sure ranking are the
    same for \pzero or \pone configurations.
    Consider a configuration $(v,m)$ in $G\times M$ and the matching
    $(\overline{v},m)$ in $G'\times M$.

    \begin{itemize}
    \item
      Suppose that $v$ is such that $p(v)$ is even.
      We set the ranking $r$ for all configurations in the gadget
      replacing $v$ to $r(v)$.
      By definition~\ref{def:almost-sure ranking} for $v$ we know that
      either 
      $\prob{v}{\vec{r}_{\leq_{p(v)-1}}}=1$ or there is some odd $j$
      such that $\prob{v}{\vec{r}_{\leq_{j-2}}}=1$ and
      $\prob{v}{\vec{r}_{<j}}\geq \epsilon$.
      \begin{itemize}
      \item
        In the first case,
        from $\overline{v}$ and for every $i$ we know that
        $r(\overline{v})\geq_{p(v)-1} r(\tilde{v},2i)$.
        Similarly, for $(\tilde{v},2i)$ we know that $r(\tilde{v},2i)
        \geq_{p(v)-1} r(\hat{v},2i)$.
        Finally, as $p(\hat{v},2i)=2i$ and for every successor $w$ we are
        ensured that $r(\hat{v},2i)\geq_{p(v)-1}r(w)$, which implies that
        $r(\hat{v},2i)\geq_{2i-1} r(w)$.
        It follows, that for every \pone configuration in the gadget we
        have that the ranking does not increase for its parity for all
        successors and for \pzero configurations there is a successor
        such that the ranking does not increase.
      \item
        In the second case, let $j$ be the minimal odd number such that 
        $\prob{v}{\vec{r}_{\leq_{j-2}}}=1$ and
        $\prob{v}{\vec{r}_{<j}}\geq \epsilon$.
        It follows that there is some successor $w$ for which
        $\vec{r}(w) <_j \vec{r}(v)$.
        
        As before, from $\overline{v}$ and for every $i$ we know that
        $r(\overline{v})\geq_{p(v)-1} r(\tilde{v},2i)$.
        For $(\tilde{v},2i)$ such that $2i<j$ we know that
        $r(\tilde{v},2i)\geq_{p(v)-1}r(\hat{v},2i)$.
        For $(\tilde{v},2i)$ such that $2i>j$ we know that
        $r(\tilde{v},2i)\geq_{p(v)-1}r(\hat{v},2i-1)$.
        Finally, for $i<j$ we know that for all successors $w$ of $v$ we
        have $r(v)\geq_{j-2}r(w)$.
        It follows that $r(\hat{v},2i)\geq_{2i}r(w)$.
        For $i\geq j$ we know that for some successor $w$ of $v$ we have
        $r(v)>_{j}r(w)$.
        It follows that $r(\hat{v},2i-1)>_{2i-1}r(w)$.
      \end{itemize}
    \item
      Suppose that $v$ is such that $p(v)$ is odd.
      We set the ranking $r$ for all configurations in the gadget
      replacing $v$ to $r(v)$.
      By definition~\ref{def:almost-sure ranking} for $v$ we know that
      there is some odd $j$ such that 
      $\prob{v}{\vec{r}_{\leq_{j-2}}}=1$ and
      $\prob{v}{\vec{r}_{<j}}\geq \epsilon$.

      Let $j$ be the minimal odd number such that  
      $\prob{v}{\vec{r}_{\leq_{j-2}}}=1$ and
      $\prob{v}{\vec{r}_{<j}}\geq \epsilon$.
      It follows that there is some successor $w$ for which
      $\vec{r}(w) <_j \vec{r}(v)$.
        
      As before, from $\overline{v}$ and for every $i$ we know that
      $r(\overline{v})\geq_{p(v)-1} r(\tilde{v},2i)$.
      For $(\tilde{v},2i)$ such that $2i<j$ we know that
      $r(\tilde{v},2i)\geq_{p(v)-1}r(\hat{v},2i)$.
      For $(\tilde{v},2i)$ such that $2i>j$ we know that
      $r(\tilde{v},2i)\geq_{p(v)-1}r(\hat{v},2i-1)$.
      Finally, for $i<j$ we know that for all successors $w$ of $v$ we
      have $r(v)\geq_{j-2}r(w)$.
      It follows that $r(\hat{v},2i)\geq_{2i}r(w)$.
      For $i\geq j$ we know that for some successor $w$ of $v$ we have
      $r(v)>_{j}r(w)$.
      It follows that $r(\hat{v},2i-1)>_{2i-1}r(w)$.
    \end{itemize}      

    It follows that $r$ induces a good parity ranking on $G'\times M$.
    Then, \pzero wins in $G'\times M$ according to $W_{as}$.
  \end{proof}
}

\begin{figure*}[bt]
  %resizebox{width=\linewidth}{
  \input{figures/gadget.tex}
  %}
  \vspace*{-7mm}
  \caption{Gadget to replace probabilistic configurations in reduction for a
    configuration with odd parity.}
  \label{figure:reduction from almost sure to sure}
  \vspace*{-4mm}
\end{figure*}

\begin{proof}
  Let $G=(V,(V_0,V_1,V_p),E,\kappa,\mathcal{W})$. 
  Let $p_{as}:V\rightarrow [0..d_{as}]$ be the
  parity ranking function that induces $W_{as}$ and $p_s:V\rightarrow
  [0..d_s]$ be the parity ranking function that induces $W_s$.
  Without loss of generality assume that both $d_s$ and $d_{as}$ are
  even.
  
  Given $G$ we construct the game $G'$ where every configuration $v\in
  V_p$ is replaced by the gadget in
  Figure~\ref{figure:reduction from almost sure to sure}. 
  That is, $G'=(V',(V'_0,V'_1),E',\kappa',\mathcal{W}')$, where the
  components of $G'$ are as follows:
  \begin{compactitem}
  \item
    $V'_0=V_0$ \hfill $\cup$
    
    $\left \{ (\tilde{v},2i), (\hat{v},2j-1) ~\left |
    \begin{array}{l}
      v\in V_p,~2i \in [0..p_{as}(v)+1], \\
      \mbox{and } 2j-1 \in [1..p_{as}(v)]
      \end{array} \right . \right \}$
  \item
    %
    $V'_1=V_1 \cup \{\overline{v}, (\hat{v},2i) ~|~ v\in V_p \mbox{
    and } 2i\in [0..p_{as}(v)]\}$
  \item
    $E'=\{ (v,w) ~|~ (v,w)\in E \cap (V_0 \cup V_1)^2 \}$ \hfill
    $\cup\hspace{19pt}$
    
    $
    \begin{array}{l l}
      \{ (v,\overline{w}) ~|~ (v,w)\in E \cap (V_0\cup V_1)\times
      V_p\} &  \cup \\
      \{ ((\hat{v},j),w) ~|~ (v,w)\in E \cap V_p \times (V_0 \cup V_1)\} &
      \cup \\
      \{ ((\hat{v},j),\overline{w}) ~|~ (v,w)\in E \cap V_p^2\} & \cup \\
      \{ (\overline{v},(\tilde{v},2i)) ~|~ v\in V_p\} & \cup \\
      \{ ((\tilde{v},2i),(\hat{v},j)) ~|~ v\in V_p \mbox{ and } j\in
        \{2i,2i-1\}\}
    \end{array}
    $
  \item
    $\mathcal{W}'=W'_{s} \cap W'_{as}$, where $W'_s$ and $W'_{as}$ are the
    parity winning sets that are induced by the following priority
    functions.
    $$
    \begin{array}{r c l}
      p'_{as}(t) & ~=~ & \left \{ 
    \begin{array}{l l}
      p_{as}(t) & t\in V_0 \cup V_1 \\
      p_{as}(v) & t \in \{\overline{v} ,(\tilde{v},2i)\} \\
      j & t=(\hat{v},j)
    \end{array} \right . \\
    p'_{s}(t) & = & \left \{
      \begin{array}{l l}
        p_s(t) & t\in V_0\cup V_1 \\
        p_s(v) & t\in \{\overline{v}, (\tilde{v},2i), (\hat{v},j)\}
      \end{array}
      \right .
    \end{array}
    $$ 
  \end{compactitem}

  We show that \pzero sure wins from a configuration $v\in V_0\cup V_1$ in $G'$
  iff she wins from $v$ in $G$ with a finite-memory strategy and she
  wins from $\overline{v}\in V'_p$ in $G'$ iff she wins from $v$ in
  $G$ with a finite-memory strategy.

  The game $G'$ is a linear game whose winning condition (for \pzero)
  is an intersection of two parity conditions.
  It is known that such games are determined and that the winning sets
  can be computed in NP$\cup$co-NP \cite{CHP07}.
  Indeed, the winning condition for \pzero can be expressed as a
  Streett condition, and hence her winning can be decided in co-NP.
  The winning condition for \pone can be expressed as a Rabin
  condition, and hence her winning can be decided in NP.
  It follows that $V'$ can be partitioned to $W'_0$ and $W'_1$, the
  winning regions of \pzero and \pone, respectively.
  Furthermore, \pzero has a finite-memory winning strategy for her
  from every configuration in $W'_0$ and \pone has a memoryless
  winning strategy for her from every configuration in $W'_1$.
  Let $\sigma'_0$ denote the winning strategy for \pzero on $W'_0$ and
  $\pi'_1$ denote the winning strategy for \pone on $W'_1$.
  Let $M$ be the memory domain used by $\sigma'_0$.
  For simplicity, we use the notation $\sigma'_0\subseteq V'\times
  M\rightarrow V'\times M$, where for every $m\in M$ and $v\in V'_0$
  there is a unique $w\in V$ and $m'\in M$ such that
  $((v,m),(w,m'))\in \sigma'$ and for every $m\in M$ and $v\in V'_1$
  and $w$ such that $(v,w)\in E'$ there is a unique $m'$ such that
  $((v,m),(w,m'))\in \sigma'_0$. 
  By abuse of notation we refer to the successor of a configuration $v$
  in $G'$ and mean either $w$ or $\overline{w}$ according to the
  context.
  
  \begin{itemize}
  \item[$\Leftarrow$]
    We show that every configuration $v\in W'_0$ that is winning for \pzero
    in $G'$ is in the winning region $W_0$ of \pzero in $G$.
    Let $G'\times M$ denote the product of $G'$ with the memory domain
    $M$, where moves from configurations in $V'_0\times M$ are restricted
    according to $\sigma'_0$.
    We construct a matching game $G\times M$ restricted to the strategy
    $\sigma_0$ that is induced by $\sigma'_0$ as follows:
    \begin{itemize}
    \item
      From a configuration $(v,m) \in V_0 \times M$ the strategy $\sigma'_0$
      chooses a successor $(w,m')$.
    \item
      From a configuration $(v,m) \in V_1 \times M$ and for every
      successor $w$ of $v$ there is a memory value $m'$ such that
      $(w,m')$ is a reachable pair of configuration and memory value in
      $G'\times M$.
    \item
      Consider a configuration $(v,m) \in V_p \times M$.
      As $\overline{v}$ is a \pone configuration in $G'$, every configuration
      $(\tilde{v},2i)$ is a possible successor of $\overline{v}$ according
      to $\sigma'_0$.
      \begin{itemize}
      \item
        If for some $i$ we have that the choice from $(\tilde{v},2i)$
        according to $\sigma'_0$ is $(\hat{v},2i-1)$.
        Then, let $i_0$ be the minimal such $i$ and let $w_0$ be the
        successor of $v$ such that the choice of $\sigma'_0$ from
        $(\hat{v},2i_0-1)$ is $w_0$.
        We update in $G\times M$ the edge from $(v,m)$ to $(w_0,m')$,
        where $m'$ is the memory resulting from taking the path
        $\overline{v}$, $(\tilde{v},2i_0)$, $(\hat{v},2i_0-1)$,
        $w_0$ in $G'\times M$.
        We update in $G\times M$ the edge from $(v,m)$ to $(w',m_{w'})$
        for $w'\neq w_0$, where $m_{w'}$ is the memory resulting from
        taking the path $\overline{v}$, $(\tilde{V},2i_0-2)$,
        $(\hat{v},2i_0-2)$, $w'$.
        Notice that as $i_0$ is chosen to be the minimal the choice
        from $(\tilde{V},2i_0-2)$ to $(\hat{v},2i_0-2)$ is compatible
        with $\sigma'_0$, where $2i_0-2$ could be $0$.
      \item
        If for all $i$ we have that the choice from $(\tilde{v},2i)$
        according to $\sigma'_0$ is $(\hat{v},2i)$.
        Then, for every $w$ successor of $v$ we update in $G\times M$
        the edge from $(v,m)$ to $(w,m')$, where $m'$ is the memory
        resulting from taking the path
        $\overline{v}$, $(\tilde{v},p_{as}(v))$, $(\hat{v},p_{as})$,
        $w$.
      \end{itemize}
      Notice that if $p_{as}(v)$ is odd then the first case always
      holds as the only successor of $(\tilde{v},p_{as}(v)+1)$ is
      $(\hat{v},p_{as}(v))$. 
    \end{itemize}
    
    The resulting game $G\times M$ (enforcing the strategy $\sigma_0$
    described above) includes no decisions for \pzero.
    Consider the winning condition $W_{s}$.
    Every path in $G\times M$ that is consistent with
    $\sigma_0$ corresponds to a path in $G'\times M$ that is consistent
    with $\sigma'_0$ and agrees on the parities of all configurations
    according to $p_{s}$.
    Indeed, every configuration of the form $(\tilde{v},2i)$ or $(\hat{v},j)$
    in $G'$ has the same priority according to $p_s$ as $\overline{v}$ (and
    $v$ in $G$).
    As every path in $G'\times M$ is winning according to $W'_s$ then
    every path in $G\times M$ is winning according to $W_s$.

    We turn our attention to consider only the parity condition
    $p_{as}$ in both $G'\times M$ and $G\times M$.
    We think about $G'\times M$ as a parity game with the winning
    condition $W'_{as}$ and about $G\times M$ as a stochastic parity
    game with the winning condition $W_{as}$.
    As $\sigma'_0$ is winning, all paths in $G'\times M$ are winning
    for \pzero according to $W'_{as}$.
    
    We recall some definitions and results from \cite{CJH04}.
    For $k\leq d_{as}$, let $\underline{k}$ denote $k$ if $k$ is odd and 
    $k-1$ if $k$ is even.
    A \emph{parity ranking} for \pzero is
    $\vec{r}:V'\times M \rightarrow [n]^{d_{as}/2}\cup \{\infty\}$ for
    some $n\in \mathbb{N}$.
    For a configuration $v$, we denote by $\vec{r}^k(v)$ the prefix 
    $(r_1,r_3,\ldots, r_{\underline{k}})$ of $r(v)$.
    Let $\vec{r}(v)=(r_1,\ldots, r_d)$ and $\vec{r}(v')=(r'_1,\ldots,
    r'_d)$.
    We write $\vec{r}(v)\leq_k\vec{r}(v')$ if the prefix
    $(r_1,\ldots r_{\underline{k}})$ is at most
    $(r'_1,\ldots, r'_{\underline{k}})$
    according to the lexicographic ordering.
    Similarly, we write $\vec{r}(v)<_k\vec{r}(v')$ if 
    $(r_1,\ldots r_{\underline{k}})$ is less than 
    $(r'_1,\ldots, r'_{\underline{k}})$
    according to the lexicographic ordering.
      
    It is well known that in a parity game (here $G'\times M$) there
    is a \emph{good} parity ranking such that for every $v \in W'_0$
    we have $\vec{r}(v)\neq \infty$ \cite{Jur00}.
    A parity ranking is good if
    \begin{inparaitem}
      \item[(i)]
        for every vertex $v\in V_0$ there is a vertex $w\in succ(v)$
        such that $\vec{r}(w)\leq_{p(v)}\vec{r}(v)$ and if $p(v)$ is
        odd then $\vec{r}(w)<_{p(v)}\vec{r}(v)$ and 
      \item[(ii)]
        for every vertex $v\in V_1$ and every vertex $w\in succ(v)$
        it holds that $\vec{r}(w)\leq_{p(v)}\vec{r}(v)$ and if $p(v)$
        is odd then $\vec{r}(w)<_{p(v)}\vec{r}(v)$.
    \end{inparaitem}
    Let $\vec{r}$ be the good parity ranking for $G'\times M$.
    Consider the same ranking for $G\times M$.
    For a configuration $v\in V_p\times M$, we write
    $\prob{v}{\vec{r}_{\leq_k}}$ for the probability 
    of successors $w$ of $v$ such that $\vec{r}(w)\leq_k \vec{r}(v)$ and
    $\prob{v}{\vec{r}_{<_k}}$ for the probability of successors $w$ of
    $v$ such that $\vec{r}(w) <_k \vec{r}(v)$.
    \begin{definition}[Almost-sure ranking \rm{\cite{CJH04}}]
      A ranking function $r:V\rightarrow [n]^{d_{as}/2}\cup \{\infty\}$ for
      \pzero is an almost-sure ranking if there is an $\epsilon\geq 0$
      such that for every vertex $v$ with $r(v)\neq \infty$, the
      following conditions hold:
      \begin{compactitem}
      \item
        If $v\in V_0$ there exists a successor $w$ such that
        $\vec{r}(w)\leq_{p(v)} \vec{r}(v)$ and if $p(v)$ is odd then
        $\vec{r}(w)<_{p(v)} \vec{r}(v)$.
      \item
        If $v\in V_1$ then for every successor $w$ of $v$ we have 
        $\vec{r}(w)\leq_{p(v)}\vec{r}(v)$ and if $p(v)$ is odd then
        $\vec{r}(w)<_{p(v)} \vec{r}(v)$.
      \item
        If $v\in V_p$ and $p(v)$ is even then either
        $\prob{v}{\vec{r}_{\leq_{p(v)-1}}}=1$
        or 
        $$
        \bigvee_{j=2i+1 \in [1..p(v)]}
        (\prob{v}{\vec{r}_{\leq_{j-2}}}=1 \wedge
        \prob{v}{\vec{r}_{<_j}}\geq \epsilon) 
        )$$ 
      \item
        If $v\in V_p$ and $p(v)$ is odd then
        $$\bigvee_{j=2i+1 \in [1..p(v)]} (\prob{v}{\vec{r}_{\leq_{j-2}}}=1 \wedge
        \prob{v}{\vec{r}_{<_j}}\geq \epsilon) $$
      \end{compactitem}
      \label{def:almost-sure ranking}
    \end{definition}
    
    \begin{lemma}{\rm \cite{CJH04}}
      A stochastic parity game has an almost-sure ranking iff \pzero
      can win for the parity objective with probability 1 from every
      configuration $v$ such that $\vec{r}(v)\neq \infty$.
      \label{lemma:almost-sure ranking}
    \end{lemma}
    
    The following lemma is a specialization of a similar lemma in
    \cite{CJH04} for our needs.
    \begin{lemma}
      The good ranking of $G'\times M$ induces an almost-sure ranking
      of $G \times M$.
      \label{lemma:good ranking induces as ranking}
    \end{lemma}

    % The actual proof is given above the beginning of the proof
    % of Theorem
    
    \shorten{
      \proofoflemmagoodrankinginduces
    }{
      We include the proof of this Lemma in Appendix.
    }
    
    As \pzero has no choices in $G\times M$, it follows that the
    strategy $\sigma_0$ defined above is winning in $G$.
    That is, sure winning according to $W_s$ and almost-sure winning
    according to $W_{as}$. 

  \item[$\Rightarrow$]

    Consider a configuration $v\in V$ such that \pzero has a
    finite-memory winning strategy in $G$ starting from $v$.
    Let the strategy be $\sigma_0$ and the memory used by $\sigma_0$
    be $M$.
    That is, there is a strategy $\sigma_0$ using finite memory domain
    $M$ such that from every configuration in $W_0$ the probability of
    winning according to $W_{as}$ is 1 and all plays are winning
    according to $W_s$.
    As before, consider the product of the game $G$ with the memory
    $M$.
    The result is a finite-state MDP.

    Consider now the imposition of the strategy $\sigma_0$ to $G'$
    using the same memory.
    We have to show how to update the memory from configurations that
    result from inclusions of the gadgets that replace probabilistic
    configurations in $G'$.
    Consider a configuration $\overline{v}$ reached with some memory
    value $m \in M$.
    In $G$ the configuration $(v,m)$ is a probabilistic configuration.
    It follows that for every successor $w$ of $v$ there is a memory
    value $m_w$ such that on transition to $w$ the memory is updated
    to $m_w$.
    We do the same in $G'$.
    That is, the memory stays $m$ while exploring the gadget with
    configurations $\overline{v}$, $(\tilde{v},2i)$, and
    $(\hat{v},j)$.
    Once the play reaches a configuration $w$ the memory is updated to
    $m_w$ as in $G$.

    The result is a parity game, which we denote by $G'\times M$. 
    As all paths in $G\times M$ are winning for \pzero according to
    the winning condition $W_s$ and the gadgets do not affect the
    winning condition $W'_s$, it follows that all plays in $G'\times
    M$ are winning according to $W'_s$ regardless of the choices of
    \pzero and \pone in the gadgets.
    We have to show that we can augment the strategy within the
    gadgets so that all plays are winning according to $W'_{as}$.

    According to Lemma~\ref{lemma:almost-sure ranking} there exists an
    almost-sure ranking $r:G\times M$.
    We show that $r$ induces a good parity ranking over $G'\times M$.

    \begin{lemma}
      The almost-sure ranking of $G\times M$ induces a good ranking of
      $G'\times M$.
      \label{lemma:good as ranking induces}
    \end{lemma}

    \shorten{
      \proofoflemmagoodasrankinginduces
    }{
      The proof is included in Appendix.
    }
    
  \end{itemize}
    
  The Theorem follows.
\end{proof}

\begin{corollary}
  Consider an SAS game with $n$ configurations, sure winning
  condition of index $d_s$, and almost-sure condition of index of
  $d_{as}$.
  Deciding whether \pzero can win with finite-memory is
  co-NP-complete.
  Deciding whether \pone can win against finite-memory is
  NP-complete.
\end{corollary}

\begin{proof}
  Upper bounds follow from the reductions to Streett and Rabin
  winning conditions.
  Completeness follows from the case where the game has no
  stochastic configurations.
\end{proof}

\begin{remark}
  The complexity established above in the case of finite-memory is the
  same as that established for the general case in
  Corollary~\ref{corollary:complexity of sas games}.
  However, this reduction gives us a clear algorithmic approach to
  solve the case of finite-memory strategies.
  Indeed, in the general case, the proof of NP upper bound requires 
  enumeration of all memoryless strategies, and does not present an 
  algorithmic approach, regardless of the indices of the different 
  winning conditions.
  In contrast our reduction for the finite-memory case to non-stochastic 
  games with conjunction of parity conditions and recent algorithmic 
  results on non-stochastic games with $\omega$-regular conditions of~\cite{CJKLS17}
  imply the following:
 \begin{compactitem} 
  \item For the finite-memory case, we have a fixed parameter tractable 
  algorithm that is polynomial in the number of the game configurations and
  exponential only in the indices to compute the SAS winning region.
  \item For the finite-memory case, if both indices are constant or 
  logarithmic in the number of configurations, we have a polynomial time algorithm to 
  compute the SAS winning region.
  \end{compactitem}
\end{remark}




==> sasmdp.tex <==
\section{Sure-Almost-Sure MDPs}
\label{section:sas MDPs}

Berthon et al.~considered the case of MDPs with two parity conditions
and finding a strategy that has to satisfy one of the conditions
surely and satisfy a given probability threshold with respect to the
other \cite{BRR17}. 
Here we consider the case that the second condition has to hold with
probability 1. 
We consider winning conditions composed of two parity conditions.
The goal of \pzero is to have one strategy such that she can win
\emph{surely} for the \emph{sure} winning condition and
\emph{almost-surely} for the \emph{almost-sure} winning condition.
The authors of \cite{BRR17} show that optimal strategies exist in
this case and that it can be decided which of the players wins.
Here we extend their results by showing that \pzero may need infinite
memory in order to win in such an MDP.
However, checking whether she can win using a finite-memory strategy
is a lot simpler than deciding if there is a general winning
strategy.

Given a set of configurations $V$, a sure-almost-sure winning
condition is $\mathcal{W}=(W_s,W_{as})$, where $W_s \subseteq V^\omega$
and $W_{as}\subseteq V^\omega$ are two parity winning conditions.
A sure-almost-sure MDP is $G=(V,(V_0,V_p),E,\kappa,\mathcal{W})$, where
all components are as before and where $\mathcal{W}$ is a
sure-almost-sure winning condition.
Strategies for \pzero are defined as before.
We say that \pzero wins from configuration $v$ if the same strategy
$\sigma$ is winning surely with respect to $W_{s}$ and almost-surely
with respect to $W_{as}$.
%for every $r<1$
%there is a strategy $\sigma_r$ such that  $v(\sigma_r)\subseteq W_s$
%and $\prob{v(\sigma_r)}{W_{as}}\geq r$.
%We say that \pzero has an optimal strategy for winning if she has a
%strategy $\sigma$ such that $v(\sigma)\subseteq W_s$ and
%$\prob{v(\sigma)}{W_{as}}=1$.

\begin{theorem}{\rm \cite{BRR17}}
  In a finite SAS parity MDP deciding whether a configuration $v$ is winning
  for \pzero is in NP$\cap$co-NP. Furthermore, there exists an optimal
  infinite-state strategy for the joint goal.
  \label{theorem:icalp theorem}
\end{theorem}

First, we show finite-memory strategies are not strong enough to
capture winning for \pzero.

\begin{theorem}
  For SAS MDPs finite-memory strategies are not strong enough to
  capture winning.
  \label{theorem:sas mdp optimal not finite}
\end{theorem}

\newcommand{\proofoftheoremsasmdpoptimalnotfinite}{
\begin{proof}
Consider the MDP in Figure~\ref{fig:mdp infinite memory}.
Here $W_s$ is induced by the B\"uchi winning condition $\{l,r\}$ and
$W_{as}$ is induced by the co-B\"uchi winning condition $\{r\}$.
That is, in order to win surely, either $l$ or $r$ has to be visited
infinitely often in every path and, in order to win almost surely,
$r$ has to be visited finitely often with probability $1$.

We show that every finite-memory strategy that wins almost-surely
with respect to $W_{as}$ is losing according to $W_s$.
Consider a finite-memory strategy $\sigma$.
Consider the Markov chain $v_0(\sigma)$.
As $\sigma$ is finite memory, $v_0(\sigma)$ is a finite-state Markov
chain.
It follows that bottom strongly connected components are reached with
probability $1$ and once a bottom SCC is reached all configurations in that SCC
are visited with probability $1$.
Suppose that $r$ appears in some reachable bottom SCC.
Then, clearly, the almost-sure winning condition cannot have the
probability $1$.
It follows that $r$ does not appear in bottom SCCs of $v_0(\sigma)$
and that in bottom SCCs the choice of \pzero from configuration $c$ is to go to
configuration $p$.
This implies that the infinite suffix $(c\cdot p)^\omega$ appears in 
$v_0(\sigma)$.
However, this path violates the sure winning condition.

We show that \pzero has an optimal strategy that uses infinite memory.
Consider the following strategy.
\pzero plays in rounds.
In the $j$-th round \pzero plays as follows.
She maintains a counter of how many times the play visited $c$ without
visiting $l$.
As long as the counter is smaller than $j$ she continues moving left
from $c$ to $p$.
Once she visits $l$ she moves to round $j+1$.
Once the counter reaches $j$ she chooses to visit $r$ by going right
from $c$ and moves to round $j+1$.
It follows that there are infinitely many rounds and in every round
parity $0$ for $W_s$ is visited.
Hence, \pzero wins surely according to $W_s$.
Furthermore, the probability to reach $r$ in the $j$-th round is
bounded by $\frac{1}{2^j}$.
Dually, the probability to not visit $r$ in the $j$-th round is at
least $1-\frac{1}{2^j}$.
So, from round $j$ onwards the probability never 
visit $r$ again is at least
$\prod_{k=j}^\infty \left( 1-\frac{1}{2^k} \right )$.
It follows that the probability to visit $r$ infinitely often is $0$.
\end{proof}
}
\shorten{
  \proofoftheoremsasmdpoptimalnotfinite
}{
  In Appendix we show that in the MDP in Figure~\ref{fig:mdp infinite
    memory} there is an infinite-memory strategy that can win both the
  sure (visit $\{l,r\}$ infinite often) and almost-sure (visit $\{r\}$
  finitely often) winning conditions.
  On the other hand, every finite-memory strategy that wins
  almost-surely is losing the sure winning condition.
}

\begin{figure}[bt]
  \input{figures/mdp.tex}
  \caption{%
    \label{fig:mdp infinite memory}%
    An MDP where \pzero requires infinite memory to win. Configuration $p$
    is probabilistic and configurations $l$, $c$, and $r$ are \pzero
    configurations. The parity is induced by the following priorities
    $\alpha_s(l)=\alpha_s(r)=0$, $\alpha_s(p)=\alpha_s(c)=1$, and
    $\alpha_{as}(r)=1$ and
    $\alpha_{as}(l)=\alpha_{as}(c)=\alpha_{as}(p)=2$.
  }
\end{figure}

We now show a chain of reductions that reduces the check of whether an
SAS MDP has a winning finite-memory strategy to deciding the winner
in a (non-stochastic) parity game.

\begin{theorem}
  In order to decide whether it is possible to win an SAS MDP with $n$
  locations and indices $d_s$ and $d_{as}$ with finite memory it is
  sufficient to solve a parity game with $O(n\cdot d_{s}\cdot d_{as})$
  configurations and index $d_{s}$. Furthermore, $d_s$ is a bound on
  the size of the required memory in case of a win.
  \label{theorem:mdp finite memory}
\end{theorem}

The theorem follows from the following Lemmas. 

\begin{lemma}
  Given an SAS MDP $M$ with $n$ configurations and almost-sure index
  of $d_{as}$, checking whether
  \pzero has a finite-memory winning strategy can be reduced to
  checking whether \pzero has a finite-memory winning strategy in an SAS MDP
  $M'$ with $O(n\cdot d_{as})$ configurations, where the almost-sure
  winning condition is a B\"uchi condition and the sure winning
  condition has the same index.
  \label{lemma:sas mdp to buchi sas mdp}
\end{lemma}

\newcommand{\proofoflemmasasmdptobuchisasmdp}{
\begin{proof}
  Consider an MDP
  $G=(V,(V_0,V_p),E,\kappa,\mathcal{W})$, where $\mathcal{W}=(W_s,W_{as})$.
  Suppose that there is an winning finite-memory strategy $\sigma$ for
  $G$.
  Let $\sigma$ be composition of $\sigma_s$ and $\sigma_u$, where
  $M=\{1,\ldots, m\}$ is the memory domain used by $\sigma$.
  Then, the Markov chain $G^M=(M\times V,V^M_p,E^M,\kappa^M,\mathcal{W}^M)$,
  where 
  $E^M=\{((m,v),(m',v')) ~|~ (v,v')\in E \mbox{ and }m'=\sigma_u(m,v')\}$,
  for $(m,v)$ such that $v\in V_p$ we have $\kappa^M$ induced by
  $\kappa$ in the obvious way and for $(m,v)$ such that $v\in V_0$ we
  have $\kappa^M$ induced by $\sigma_s(m,v)$.
  The condition $\mathcal{W}^M$ is obtained by considering the projection
  of a play on $V^\omega$.
  Clearly, $G^M$ is a finite-state Markov chain.
  It follows that in $G^M$ bottom SCCs are reached with probability $1$ 
  and in every bottom SCC every configuration is visited infinitely
  often with probability $1$.
  Consider a bottom SCC in $G^M$. There is some minimal parity
  appearing in this bottom SCC, which will be visited infinitely
  often.
  It follows that we can consider this minimal parity as a B\"uchi
  condition.
  We reduce the optimal winning with finite-memory in $G$ to the
  optimal winning with finite-memory in an MDP $G'$, where the
  almost-sure winning condition is a B\"uchi condition and the sure
  winning condition has the same index.

  Formally, we have the following.
  Let $\alpha_{as}:V \rightarrow \{0,\ldots, 2d_{as}\}$ be the parity
  function inducing $W_{as}$ and let $\alpha_s:V\rightarrow
  \{0,\ldots, 2d_{s}\}$ be the parity function inducing $W_s$. 
  Let $G_b=(V',(V'_0,V'_p),E',\kappa',\mathcal{W'})$, where $G_b$ has the
  following components. For a set $V$ let $\tilde{V}$ denote the set
  $\{\tilde{v} ~|~ v\in V\}$. 
  \begin{itemize}
  \item
    $V' = V \cup \tilde{V} \cup V \times \{0,2,\ldots, 2d_{as}\} \cup \{\bot\}$
  \item
    $V'_0 = V_0 \cup \tilde{V} \cup V_0 \times \{0,2,\ldots, 2d_{as}\}$
  \item
    $V'_p = V'\setminus V'_0$
  \item
    $E'= \{ (v,\tilde{w}) ~|~ (v,w)\in E \} \cup \{(\bot,\bot)\}$
    \shorten{\hfill}{} $\cup\hspace{5pt}$

    \shorten{\hfill}{} $
    \begin{array}{l r}
          \{(\tilde{v},(v,i)), (\tilde{v},v),(\tilde{v},\bot) ~|~ v\in
          V \}  & \cup \\
      \{((v,i),(w,i)) ~|~ (v,w) \in E \mbox{ and } \alpha_{as}(v) \geq
      i \}
      &
      \cup \\
      \{((v,i),\bot) ~|~ \alpha_{as}(v) < i \} 
    \end{array}
    $
  \item
    For $v\in V_p$ we have 
    $\kappa'(v,\tilde{w}) = \kappa'((v,i),(w,i)) = \kappa(v,w)$
    and
    $\kappa'((v,i),\bot) = 1$.
  \item
    $\mathcal{W}' = (W'_s,W'_{as})$, where $W'_s$ is induced 
    by $\alpha'_s(q)=\alpha'_s(\tilde{q})=\alpha'_s(q,i)=\alpha_s(q)$ and
    $\alpha_s(\bot)=1$ and $W'_{as}$ is induced by $\alpha'_{as}$
    where $\alpha'_{as}(q,i) = 0$ if $\alpha_{as}(q)=i$ and
    $\alpha'_{as}$ is $1$ for all other configurations.
  \end{itemize}

  The MDP $G_b$ has an original (extended) copy of $G$ and additional
  $d_{as}+1$ restricted copies of $G$.
  In the original copy ($V\cup \tilde{V}$), every move in $G$ is
  mimicked by two moves in $G_b$.
  Before getting to a location in $V$ we pass through a location in
  $\tilde{V}$, where \pzero is given a choice between progressing to
  $V$ (and effectively staying in the original copy) or moving on to one
  of the restricted copies (or giving up by going to $\bot$).
  Each of the other $d_{as}+1$ copies corresponds to a bottom strongly
  connected component where moves are restricted by some priority.
  Thus, in the $2i$-th copy, it is impossible to move to locations with
  parity lower than $2i$ (this is an immediate loss for \pzero), and
  the locations of parity $2i$ are B\"uchi locations.
  
  Given a finite-memory winning strategy in $G$ it can be extended to
  a finite-memory winning strategy in $G_b$ by making \pzero move to
  configurations of the form $(q,i)$ when reaching a bottom SCC whose
  minimal parity is $i$. By $i$ being the minimal parity in the bottom
  SCC, transitions to $\bot$ will not appear. The sure winning
  condition does not change.
  In the other direction, a finite-memory strategy in $G_b$ ensures
  that all bottom  SCCs visit the B\"uchi configurations infinitely
  often. Thus, for every bottom SCC there is an $i$ such that the SCC
  is composed only of configurations of the form $(q,i)$. There must be some
  state $(q',i)$ such that $\alpha_{as}(q')=i$.
  Furthermore, $\bot$ cannot be visited (as the strategy is winning)
  and hence the transitions in the SCC correctly reflect all possible
  transition in the same SCC in $G$.
\end{proof}
}
\shorten{
  \proofoflemmasasmdptobuchisasmdp
}{
  In Appendix we show that we can think about bottom SCCs where the
  almost-sure parity condition holds as a B\"uchi condition involving
  a commitment not to visit lower parities and to visit a minimal
  even parity infinitely often.
}

\begin{lemma}
  The finite-memory winning in an SAS MDP where the almost sure
  winning condition is 
  a B\"uchi condition can be checked by a reduction to a
  (non-stochastic) game where the winning condition is the
  intersection of parity and B\"uchi conditions. 
  \label{lemma:buchi sas mdp to parity and buchi}
\end{lemma}

This Lemma is an instantiation of the result in 
Theorem~\ref{theorem:sas games finite memory} for the case of
almost-sure B\"uchi.
In both cases, the proof is a version of 
the classical reduction from stochastic parity games to parity games
\cite{CJH04}.
We include the proof of this lemma in Appendix for completeness of
presentation.

\newcommand\proofoflemmabuchisasmdptoparityandbuchi{
\begin{proof}
  Consider an MDP $G=(V,(V_0,V_p),E,\kappa,\mathcal{W})$, where
  $\mathcal{W}=(W_s,W_{as})$ is such that $W_{as}$ is a B\"uchi
  condition.
  Let $B\subseteq V$ denote the set of B\"uchi configurations of the
  almost-sure winning condition.
  Let $p_s:V\rightarrow [1..d_s]$ be the parity ranking function that
  induces $W_s$.
  We create the (non-stochastic) game $G'$ by replacing every configuration
  $v\in V_p$ by one of the gadgets in Figure~\ref{figure:reduction
    from almost sure to sure mdp}.
  Formally, $G'=(V',(V'_0,V'_1),E,\mathcal{W'})$, where the components of
  $G'$ are as follows:
  \begin{itemize}
  \item
    $V'_0 = V_0 \cup \{ (\tilde{v},0), (\tilde{v},2),(\hat{v},1) ~|~
    v\in V_p\}$
  \item
    $V'_1 = \{\overline{v}, (\hat{v},0) ~|~ v\in V_p\}$
  \item
    $E'=\{ (v,w) ~|~ (v,w)\in E \cap (V_0\times V_0)\}$ \shorten{\hfill}{} $\cup\hspace{1pt}$

    $
    \begin{array}{l l}
    \{ (v,\overline{w}) ~|~ (v,w)\in E \cap (V_0 \times V_p) \} & \cup \\
    \{ ((\hat{v},i),w) ~|~ (v,w)\in E \cap (V_p \times V_0)\} & \cup \\
    \{ ((\hat{v},i),\overline{w}) ~|~ (v,w)\in E \cap (V_p \times V_p)\} & \cup \\
    \{ (\overline{v},(\tilde{v},0)),%(\overline{v},(\tilde{v},2)),
        ((\tilde{v},0),(\hat{v},0)), ((\tilde{v},2),(\hat{v},1)) ~|~
        v\in V_p \}  & \cup \\
      \{ (\overline{v},(\tilde{v},2)) ~|~ v\in
      V_p\cap B\}
    \end{array}
    $
  \item
    $\mathcal{W'}$ is the winning condition resulting from the
    conjunction (intersection) of the B\"uchi condition $V_0\cap B
    \cup \{(\hat{v},0) ~|~ v\in V_p\}$ and the parity condition
    induced from $\alpha':V'\rightarrow [1..d_s]$, where
    $\alpha'(v)=\alpha_{s}(v)$ for $v\in V_0$ and
    $\alpha'(\overline{v})=\alpha'(\tilde{v},i)=\alpha'(\hat{v},i)=\alpha_s(v)$.
  \end{itemize}

  \begin{figure}[bt]
    \input{figures/gadgetmdp.tex}
    \vspace*{-7mm}
    \caption{\label{figure:reduction from almost sure to sure mdp}%
      Gadget to replace probabilistic configurations in the reduction.}
  \vspace*{-4mm}
  \end{figure}

  We show that if \pzero has a finite-memory winning strategy in $M$
  she wins in $G$.
  Consider the combination of the winning strategy for \pzero in $M$
  with $M$.
  It follows that every bottom SCC is winning according to both $W_s$
  and $W_{as}$.
  We define the following strategy in $G'$ that uses the same memory.
  We have to extend the strategy by a decision from configurations of the form
  $(\hat{v},1)$, which belong to \pzero in $G'$.
  If the configuration $(\hat{v},1)$ is in a bottom SCC, \pzero chooses the
  successor of $v$ that minimizes the distance to $B$.
  By assumption every bottom SCC has some configuration in $B$
  appearing in it.
  If the configuration $(\hat{v},1)$ is in a non-bottom SCC, \pzero chooses the
  successor of $v$ with minimal distance to exit the SCC.
  Consider a play consistent with this strategy.
  Clearly, this play is possible also in the MDP $G$. By assumption
  the play satisfies $\alpha_s$.
  If a play visits infinitely often configurations of the type $(\hat{v},0)$,
  then this play satisfies the B\"uchi winning condition.
  Consider a play that visits finitely often configurations of the type
  $(\hat{v},0)$.
  It follows that whenever it visits a configuration of the type $\overline{v}$
  the distance to leave non-bottom SCC decreases and hence the play
  eventually reaches a bottom SCC.
  Similarly, after reaching a bottom SCC whenever a configuration of the type
  $\overline{v}$ is visited the distance to $B$ decreases.

  We show that if \pzero wins the game $G'$ she has a finite-memory
  winning strategy in $M$.
  As $G'$ does not have stochastic elements and as the winning
  condition there is $\omega$-regular, \pzero has a finite-memory pure
  winning strategy.
  In case that from $\overline{v}$ \pone chooses the successor
  $(\tilde{v},0)$ then the strategy instructs \pzero what to do from
  every successor of $v$.
  In case that from $\overline{v}$ \pone chooses the successor
  $(\tilde{v},2)$ then the strategy instructs \pzero to choose a
  unique successor of $v$.
  The strategy of \pzero in $M$ follows the strategy of \pzero in $G$.
  Whenever after a configuration $v\in V_p$ we discover that the
  successor is the one that is consistent with the choice from
  $(\hat{v},1)$ we update the memory accordingly.
  Whenever after a configuration $v\in V_p$ we discover that the
  successor is not consistent with the choice from $(\hat{v},1)$ we
  update the memory according to the choice from $(\hat{v},0)$.

  Consider a play in $M$ consistent with this strategy. Clearly, a
  version of this play appears also in $G$.
  As both the game and the MDP agree on $W_s$ and the strategy in $G$
  is winning it follows that $W_s$ is satisfied in $M$ as well.
  Consider now the winning condition $W_{as}$.
  If the play visits only finitely many configurations in $V_p$ then
  it is identical to the play in $G$ and satisfies also $W_{as}$.
  If the play visits infinitely many configurations in $V_p\cap B$
  then it is clearly winning according to $W_{as}$.
  Otherwise, the play visits infinitely many configurations in $V_p$
  but only finitely many in $V_p\cap B$.
  The play cannot stay forever in a non-bottom SCC of $G$ (combined
  with the strategy of \pzero).
  Indeed, there is a non-zero probability for the probabilistic
  choices to agree with the strategy of \pzero and leave this
  non-bottom SCC.
  Similarly, when reaching a bottom SCC, as all configurations of the
  SCC will be visited with probability 1 and from the strategy being
  winning in $G'$ we conclude that there is a configuration in $B$
  appearing in this bottom SCC and it will be visited infinitely
  often. 
\end{proof}
}

%\proofoflemmabuchisasmdptoparityandbuchi

The following Lemma is probably folklore.
However, we could not find a source for it and include it here with a
proof. 

\begin{lemma}
  A game with a winning condition that is the conjunction of B\"uchi
  and parity can be converted to an ``equivalent'' parity game.
  \label{lemma:buchi and parity to parity}
\end{lemma}

\newcommand{\proofoflemmabuchiandparitytoparity}{
\begin{proof}
  Let the parity condition be induced by the priority function
  $\alpha:V\rightarrow [0..d]$ and let the B\"uchi condition be
  $B\subseteq V$.
  For a parity $p$ let %$\lfloor p \rfloor$ denote $p$ if $p$ is even
  %and $p-1$ otherwise and let
  $\lceil p \rceil$ denote $p$ if $p$ is odd and $p+1$ otherwise.
  We take the product of the game with the deterministic monitor
  $M=(V,\{0,\ldots,\lceil d\rceil\} \times \{\bot,\top\},\delta,\alpha')$,
  where $\alpha'(i,\top)=i$ and 
  $\alpha'(i,\bot) = \lceil i \rceil$ and $\delta$ is defined as
  follows.
  We note that the monitor ``reads'' the configuration of the game.
  
  $$
  \delta((i,\beta),v) = \left \{
  \begin{array}{l l}
    (\alpha(v),\top) & v \in B \mbox{ or } \alpha(v) < i \\
    (i,\bot) & v\notin B \mbox{ and } \alpha(v) \geq i\\
  \end{array}
  \right .
  $$

  That is, the monitor memorizes the lowest parity that has been seen
  since a visit to the B\"uchi set.
  The monitor signals a ``real'' visit to parity $i$ whenever its
  second component is $\top$.
  The second component can become $\top$ whenever a B\"uchi state is
  visited or when the visited priority is lower than all priorities
  visited since the last visit to the B\"uchi set.
  
  Consider a play $p$ in $G$ that is winning according to both the
  B\"uchi condition and the original parity condition.
  Let $e$ be the least (even) parity to be visited infinitely often in
  $p$ according to $\alpha$.
  Let $j$ be the index such that $p_i$ is a visit to $B$ and after $j$
  there are no visits to parities smaller than $e$.
  Then, for every $j'\geq j$ there is a $j''\geq j$ such that $p_{j''}\in
  B$.
  If $p_{j''}$ also has parity $e$ then the state of the monitor after
  reading $p_{j''}$ is $(e,\top)$.
  If $p_{j''}$ has parity greater than $e$ then let $j'''>j''$ be the minimal
  such that $p_{j'''}$ has parity $e$.
  Then the state of the monitor after reading $p_{j'''}$ is
  $(e,\top)$.
  It follows that $(e,\top)$ is visited infinitely often.
  Also, from the structure of the monitor, the only way that the
  monitor signals a parity smaller than $e$ is if parities smaller
  than $e$ are visited in the game.
  It follows that the monitor signals acceptance.

  Consider a play $p$ in $G$ for which the minimal parity indicated by
  $\alpha'$ to be visited infinitely often is even.
  The only states of the monitor for which $\alpha'(\cdot)$ is even
  are of the form $(i,\top)$.
  States of the form $(i,\top)$ can appear at most $d/2$ times without
  a visit to a configuration in $B$, indeed, without a visit to $B$
  $i$ can only decrease.
  It follows that $p$ visits $B$ infinitely often.
  Let $e$ be the least (even) parity to be visited infinitely often in
  $p$ according to $\alpha'$.
  Let $j$ be the location such that for every $j'\geq j$ we have
  $\alpha'(\cdot) \geq e$.
  By the structure of the monitor, for every $j'>j$ we have
  $\alpha'(\cdot)$ has parity at least $e$.
  Furthermore, the only way for $\alpha'(\cdot)$ to signal parity $e$
  is after a visit to a state $p_{j''}$ for which $\alpha(p_{j''})=e$.
  It follows that $B$ is visited infinitely often and that the minimal
  parity to be visited infinitely often is even.
\end{proof}
}
\shorten{
  \proofoflemmabuchiandparitytoparity
}{
  In Appendix we show that we can add to the game a monitor that
  allows to refresh the best parity priority from one condition that
  is seen every time that the B\"uchi set from the other condition is
  visited.
}


Based on Lemmas~\ref{lemma:sas mdp to buchi sas mdp}, 
\ref{lemma:buchi sas mdp to parity and buchi}, and
\ref{lemma:buchi and parity to parity}, we can prove
Theorem~\ref{theorem:mdp finite memory}.

\newcommand{\proofoftheoremmdpfinitememory}{
\begin{proof}
  Starting from an SAS MDP with $n$ configurations, $d_s$ priorities
  in the sure winning condition and $d_{as}$ priorities in the
  almost-sure winning condition the reductions produce the following
  games.

  The reduction in Lemma~\ref{lemma:sas mdp to buchi sas mdp} produces
  an MDP with $O(n\cdot d_{as})$ configurations with a parity condition with
  $d_s$ priorities and a B\"uchi condition.

  The reduction in Lemma~\ref{lemma:buchi sas mdp to parity and buchi}
  multiples the number of configurations by at most four.
  The resulting game has a winning condition that is the intersection
  of a parity condition of index $d_{s}$ and a B\"uchi condition.
  The number of configurations remains $O(n\cdot d_{as})$.

  Finally, the reduction in
  Lemma~\ref{lemma:buchi and parity to parity} produces a parity game
  with $O(n\cdot d_{as}\cdot d_s)$ configurations and $d_s$ priorities.

  A winning strategy in the parity game is memoryless.
  This translated to a strategy with memory $d_s$ in the SAS MDP where
  the almost-sure condition is a B\"uchi condition.
  In order to use this strategy in the original SAS MDP no additional
  memory is required.

  It follows that in order to decide whether it is possible to win an SAS MDP with
  indices $d_s$ and $d_{as}$ with finite memory we can solve a parity
  game with $O(n \cdot d_{as}\cdot d_s)$ configurations and a memory
  of size $d_{s}$ is sufficient.
\end{proof}
}

\proofoftheoremmdpfinitememory

\begin{corollary}
  Consider an SAS MDP with $n$ configuration, sure winning
  condition of index $d_s$, and almost-sure winning condition of index $d_{as}$.
  Checking whether \pzero can win with finite-memory can be computed
  in quasi-polynomial time.
  In case that $d_s \leq \log{n}$ it can be decided in polynomial
  time. 
\end{corollary}

\begin{proof}
  This is a direct result of Theorem~\ref{theorem:mdp finite memory}
  and the quasi-polynomial algorithm for solving parity games in \cite{CJKLS17,JL17}.
\end{proof}


==> sls.tex <==
\section{Sure-Limit-Sure Parity Games}
\label{section: sls games}

In this section we extend our results to the case where the unsure goal
is required to be met with limit-sure certainty, rather than almost-sure
certainty.


\smallskip\noindent{\em Sure-limit-sure parity games.}
A {\em sure-limit-sure (SLS) parity game} is, as before,
$G=(V,(V_0,V_1,V_p), E,\kappa,\mathcal{W})$.
We denote the second winning condition with the subscript $ls$, i.e.,
$W_{ls}$.
We say that \pzero wins $G$ from configuration $v$ if she has a sequence 
of strategies $\sigma_i\in \Sigma$ such that for every $i$ for every strategy 
$\pi$ of \pone we have
$v(\sigma_i)\subseteq W_s$ and 
$\prob{v(\sigma_i,\pi)}{W_{ls}}\geq 1-\frac{1}{i}$.
That is, \pzero has a sequence of strategies that are 
sure winning (on all paths) with respect to $W_s$ and 
ensure satisfaction probabilities approaching~1 
with respect to $W_{ls}$.

\subsection{Limit-Sure vs Almost-Sure}
In MDPs and stochastic turn-based games with parity conditions almost-sure
and limit-sure winning coincide~\cite{Cha07}.
In contrast to the above result we present an example MDP where in addition
to surely satisfying one parity condition limit-sure winning with another
parity condition can be ensured, but almost-sure winning cannot be ensured.
In other words, in conjunction with sure winning, limit-sure winning does not 
coincide with almost-sure winning even for MDPs.


\begin{theorem}
  While satisfying one parity condition surely, winning limit-surely with respect to another 
  parity condition is strictly stronger than wining almost-surely.
  This holds true already in the context of MDPs.
\end{theorem}

\begin{proof}
  Consider the MDP in Figure~\ref{fig:sls mdp}. 
  Clearly, \pzero wins surely with respect to both parity conditions
  in configuration $r$.
  In order to win $W_s$ the cycle between $p$ and $c$ has to be taken 
  finitely often.
  Then, the edge from $c$ to $l$ must be taken eventually.
  However, $l$ is a sink that is losing with respect to $W_{ls}$. 
  It follows, that \pzero cannot win almost-surely with respect to $W_{ls}$ 
  while winning surely with respect to $W_s$.
  
  On the other hand, for every $\epsilon>0$ there is a finite-memory strategy that is 
  sure winning with respect to $W_s$ and wins with probability at least $1-\epsilon$ with
  respect to $W_{ls}$.
  Indeed, \pzero has to choose the edge from $c$ to $p$ at least $N$ times,
  where $N$ is large enough such that $\frac{1}{2^N}<\epsilon$, and then
  choose the edge from $c$ to $l$.
  Then, \pzero wins surely with respect to $W_s$ (every play eventually
  reaches either $l$ or $r$) and wins with probability more than $1-\epsilon$ 
  with respect to $W_{ls}$. 
\end{proof}

\begin{figure}[bt]
  \input{figures/sls.tex}
  \caption{%
    \label{fig:sls mdp}%
    An MDP where \pzero can ensure sure winning and win limit-surely 
    but cannot win almost-surely.
    Configuration $p$ is probabilistic and configurations $l$, $c$, and $r$ are \pzero
    configurations. The winning conditions are induced by the following priorities
    $\alpha_s(l)=\alpha_s(r)=0$, $\alpha_s(p)=\alpha_s(c)=1$, and
    $\alpha_{ls}(r)=0$ and
    $\alpha_{ls}(l)=\alpha_{ls}(c)=\alpha_{ls}(p)=1$.
  }
\end{figure}

\subsection{Solving SLS Games}
We now present the solution to winning in SLS games, which is achieved in 
two parts: (a)~first, solve the SAS component, and (b)~then compute  
limit-sure reachability to the SAS-winning region, while respecting the 
sure parity condition.
The memory used in the SLS part has to match the memory used for
winning in the SAS part.
That is, if \pzero is restricted to finite-memory in the SAS part of
the game she has to consider finite-memory strategies in the SLS part.


\smallskip\noindent{\em SAS winning region $A$.}
Consider a game $G=(V,(V_0,V_1,V_p),E,\kappa,\mathcal{W})$, where 
$\mathcal{W}=(W_s,W_{ls})$.
Consider $G$ as an SAS game and compute the set of configurations
from which \pzero can win $G$.
Let $A\subseteq V$ denote this winning region and $B= V \setminus A$ be 
the complement region.
Clearly, $A$ is {\em closed} under \pone moves and under probabilistic
moves.
That is, if $v\in (V_1\cup V_p)\cap A$ then for every $v'$ such 
that $(v,v')\in E$ we have $v'\in A$.
Furthermore, under \pzero's winning strategy, \pzero does not use
edges going back from $A$ to $B$.
It follows that we can consider $A$ as a sink in the game $G$.


\smallskip\noindent{\em Reduction to limit-sure reachability.}
Consider a memoryless optimal strategy $\pi\in\Pi$ (we have already established 
that \pone has an optimal memoryless strategy on all her winning region) 
for the region $B$.
We present the argument for finite-memory strategies for \pzero, and the 
argument for infinite-memory strategies is similar.
Consider an arbitrary finite-memory strategy $\sigma\in \Sigma$, and consider 
the Markov chain that is the result of restricting \pzero and \pone moves 
according to $\sigma$ and $\pi$, respectively.
\begin{compactitem}
\item {\em Bottom SCC property.}
Let $S$ be a bottom SCC that intersects with $B$ in the Markov chain. 
As explained above, it cannot be the case that this SCC intersects $A$ 
(since we consider $A$ as sink due to the closed property). 
Thus the SCC $S$ must be contained in $B$.
Thus, either $S$ must be losing according to $W_s$ or the minimal 
parity in $S$ according to $W_{ls}$ is odd, as otherwise in the region $S$
\pzero ensures sure winning wrt $W_s$ and almost-sure winning wrt $W_{ls}$
against an optimal strategy $\pi$, which means that $S$ belongs to the SAS 
winning region $A$. This contradicts that $S$ is contained in $B$.

\item {\em Reachability to $A$.}
In a Markov chain bottom SCCs are reached with probability~1, and from above 
item it follows that the probability to satisfy the $W_{ls}$ goal along with 
ensuring $W_s$ while reaching bottom SCCs in $B$ is zero.
Hence, the probability to satisfy $W_{ls}$ along with ensuring $W_s$ is at most 
the probability to reach $A$.
On the other hand, after reaching $A$, the SAS goal can be ensured by switching 
to an appropriate SAS strategy in the winning region $A$, which implies that the SLS 
goal is ensured. 
Hence it follows that the SLS problem reduces to limit-sure reachability to $A$, 
while ensuring the sure parity condition $W_s$.
\end{compactitem}

\begin{remark}
Note that for finite-memory strategies the argument above is based on bottom SCCs.
Given the optimal strategy $\pi \in \Pi$, we have an MDP, and the SAS region 
for MDPs wrt to infinite-memory strategies is achieved by characterizing certain 
strongly connected components (called Ultra-good end-components~\cite[Definition~5]{BRR17}), 
and hence a similar argument as above also works for infinite-memory strategies 
to show that SLS for infinite-memory strategies for two parity conditions reduces 
to limit-sure reachability to the SAS region while ensuring the sure parity condition
(however, in this case the SAS region has to be computed for infinite-memory strategies).
\end{remark}


\smallskip\noindent{\em Limit-sure reachability and sure parity.}
Consider an SLS game, with a set $T$ of sink target states, such that the limit-sure 
goal is to reach $T$, and every state in $T$ has even priority with respect to $W_s$.
As argued above, the general SLS problem can be reduced to the limit-sure reachability 
and sure parity problem after computing the SAS region $A$ (which can be treated as 
the absorbing sink $T$).
We now present solution to this limit-sure reachability with sure parity problem.
The computational steps are as follows:
\begin{compactitem}
\item First, compute the sure winning region $X$ in the game. Note that $T \subseteq X$ as 
$T$ represent sink states with even priority for $W_s$. 
\item Second, restrict the game to $X$ and compute limit-sure reachability region to $T$, 
and let the region be $Y$.
Note that the game restricted to $X$ is a turn-based stochastic game where almost-sure and 
limit-sure reachability coincide.
\end{compactitem}
Let us denote by $Z$ the desired winning region (i.e., from where sure parity can be ensured
along with limit-sure reachability to $T$).
We argue the correctness proof that $Y$ computes the desired winning region $Z$ as follows:
\begin{compactitem}
\item First, note that since the sure parity condition $W_s$ must be ensured, the sure winning 
region $X$ must never be left. Thus without loss of generality, we can restrict the game to $X$. 
Since $Y$ is the region in $X$ to ensure limit-sure reachability to $T$, clearly $Z$ 
that must ensure both limit-sure reachability as well as sure parity is a subset of $Y$.
Hence $Z \subseteq Y$.

\item Second, for any $\epsilon>0$, there is a strategy in $Y$ to ensure that $T$ is reached with 
probability at least $1-\epsilon$ within $N_{\epsilon}$ steps staying in $X$ 
(since in the subgame restricted to $X$, almost-sure reachability to $T$ can be ensured). 
Consider a strategy that plays the above strategy for $N_{\epsilon}$ steps, and if $T$ is not reached,
then switches to a sure winning strategy for $W_s$ (such a strategy exist since $X$ is never left,
and parity conditions are independent of finite prefixes).
It follows that from $Y$ both limit-sure reachability to $T$ as well as sure parity condition 
$W_s$ can be ensured.
Hence $Y \subseteq Z$. 
\end{compactitem}
It follows from above that to solve SLS games, the following computation steps are sufficient:
(i)~solve SAS game, (ii)~compute sure winning region for parity conditions, and 
(iii)~compute almost-sure (=limit-sure) reachability in turn-based stochastic games.
The second step is a special case of the first step, and the third step can be achieved in 
polynomial time~\cite{dAHK98}.
Hence it follows that all the complexity and algorithmic upper bounds we established for 
the SAS games carries over to SLS games.
Moreover, as the complexity lower bound results for SAS parity games follow 
from games with no stochastic transitions, they apply to SLS parity games as well.
Hence we have the following corollary. 


\begin{corollary}
All complexity and algorithmic results established in Section~\ref{section:sas games} 
(resp., Section~\ref{section:sas MDPs}) for SAS turn-based stochastic 
parity games (resp., MDPs) also hold for SLS turn-based stochastic parity games (MDPs).
\end{corollary}


 





 





